HST NIR Snapshot Survey of 3CR Radio Source Counterparts II: An Atlas and Inventory of the Host Galaxies, Mergers and Companions

We present the second part of an H-band (1.6 microns) atlas of z<0.3 3CR radio galaxies, using the Hubble Space Telescope Near Infrared Camera and Multi-Object Spectrometer (HST NICMOS2). We present new imaging for 21 recently acquired sources, and host galaxy modeling for the full sample of 101 (including 11 archival) -- an 87% completion rate. Two different modeling techniques are applied, following those adopted by the galaxy morphology and the quasar host galaxy communities. Results are compared, and found to be in excellent agreement, although the former breaks down in the case of strongly nucleated sources. Companion sources are tabulated, and the presence of mergers, tidal features, dust disks and jets are catalogued. The tables form a catalogue for those interested in the structural and morphological dust-free host galaxy properties of the 3CR sample, and for comparison with morphological studies of quiescent galaxies and quasar host galaxies. Host galaxy masses are estimated, and found to typically lie at around 2*10^11 solar masses. In general, the population is found to be consistent with the local population of quiescent elliptical galaxies, but with a longer tail to low Sersic index, mainly consisting of low-redshift (z<0.1) and low-radio-power (FR I) sources. A few unusually disky FR II host galaxies are picked out for further discussion. Nearby external sources are identified in the majority of our images, many of which we argue are likely to be companion galaxies or merger remnants. The reduced NICMOS data are now publicly available from our website (http://archive.stsci.edu/prepds/3cr/)

==> tab3.tex <==
% Table 3: FULL SAMPLE PROPERTIES

\begin{deluxetable}{lllrllrrrcrr}  
  \tabletypesize{\tiny}
  \tablecolumns{12}
  \tablewidth{0pc} 
  \renewcommand{\arraystretch}{.6}
  \tablecaption{\label{tab-props} Radio Properties of the NICMOS Snapshot Survey Sample}
  \tablehead{
    \colhead{Source} & \colhead{$z$} & \colhead{$V$} &
    \colhead{$S(178~\mathrm{MHz})^{a}$/Jy} & \colhead{log$_{10}$ P$_{178}$} &  
    \colhead{$\alpha^{a}$} & \colhead{LAS$^{b,c}$} & \colhead{PA$^{b,c}$} & \colhead{FR$^{a}$} &
    \colhead{Class$^{d}$} & \colhead{$L_{OII}^{d}$} & \colhead{$L_{OIII}^{d}$}}
  \startdata
%  \input{/Users/floyd/3C/Work/idl/properties}
3C~15 & 0.073 & 15.3 & 15.8 & 26.3 & 0.64 & ... & ... & ... & ... & ... & ... \\ 
3C~17 & 0.219 & 18.0 & 20.0 & 27.4 & 0.52 & ... & ... & ... & ... & ... & ... \\ 
3C~20 & 0.174 & 19.0 & 42.9 & 27.6 & 0.67 & 51 & 101 & 2 & HEG & 33.99 & 34.47 \\ 
3C~28 & 0.195 & 17.6 & 16.3 & 27.2 & 1.06 & 30 & 166 & 2 & LEG & 35.07 & ... \\ 
3C~29 & 0.044 & 14.1 & 15.1 & 25.8 & 0.50 & 139 & 160 & 1 & ... & ... & ... \\ 
3C~31 & 0.016 & 12.1 & 16.8 & 25.0 & 0.57 & 1833 & 159 & 1 & FRI & ... & ... \\ 
3C~33 & 0.059 & 15.2 & 54.4 & 26.7 & 0.76 & ... & ... & 2 & HEG & 34.72 & 35.37 \\ 
3C~33.1 & 0.181 & 19.5 & 13.0 & 27.1 & 0.62 & 216 & 45 & 2 & WQ & ... & 35.05 \\ 
3C~35 & 0.067 & 15.6 & 10.5 & 26.1 & 0.77 & 704 & 12 & 2 & LEG & ... & ... \\ 
3C~52 & 0.285 & 18.5 & 13.5 & 27.5 & 0.62 & 51 & 20 & 2 & ... & ... & ... \\ 
3C~61.1 & 0.186 & 19.0 & 31.2 & 27.5 & 0.77 & 186 & 2 & 2 & HEG & 34.70 & 35.48 \\ 
3C~66B & 0.021 & 12.9 & 24.6 & 25.4 & 0.62 & 330 & 54 & 1 & FRI & 33.16 & 33.01 \\ 
3C~71 & 0.004 & 8.9 & 16.1 & 23.7 & 0.55 & ... & ... & ... & ... & ... & ... \\ 
3C~75N & 0.024 & 13.6 & 25.8 & 25.5 & 0.71 & 692 & 111 & 1 & ... & ... & ... \\ 
3C~76.1 & 0.032 & 14.9 & 12.2 & 25.5 & 0.77 & 200 & ... & 1 & FRI & ... & ... \\ 
3C~79 & 0.255 & 18.5 & 30.5 & 27.8 & 0.92 & 86 & 105 & 2 & WQ & 35.46 & 35.84 \\ 
3C~83.1 & 0.025 & 12.5 & 26.0 & 25.6 & 0.64 & 680 & 96 & 1 & ... & ... & ... \\ 
3C~84 & 0.017 & 11.9 & 61.3 & 25.6 & 0.78 & ... & 160 & 1 & FRI & 34.38 & 34.86 \\ 
3C~88 & 0.030 & 14.0 & 15.3 & 25.5 & 0.52 & 259 & 60 & 2 & ... & ... & ... \\ 
3C~98 & 0.030 & 14.5 & 47.2 & 26.0 & 0.78 & ... & ... & 2 & HEG & 33.53 & 34.23 \\ 
3C~105 & 0.089 & 18.5 & 17.8 & 26.5 & 0.58 & ... & 335 & 2 & ... & ... & ... \\ 
3C~111 & 0.049 & 18.0 & 64.6 & 26.6 & 0.73 & 220 & 62 & 2 & ... & ... & ... \\ 
3C~123 & 0.218 & 21.7 & 189.0 & 28.4 & 0.70 & 23 & 115 & 2 & LEG & ... & 34.98 \\ 
3C~129 & 0.021 & 19.0 & 46.9 & 25.7 & 0.92 & ... & ... & 1 & ... & ... & ... \\ 
3C~129.1 & 0.022 & 19.0 & 10.5 & 25.1 & 0.89 & ... & ... & 1 & ... & ... & ... \\ 
3C~130 & 0.109 & 16.5 & 15.5 & 26.7 & 0.89 & ... & ... & ... & ... & ... & ... \\ 
3C~132 & 0.214 & 18.5 & 13.7 & 27.3 & 0.68 & ... & ... & 2 & LEG & ... & ... \\ 
3C~133 & 0.277 & 20.0 & 22.3 & 27.7 & 0.70 & 12 & 107 & 2 & ... & ... & ... \\ 
3C~135 & 0.127 & 17.1 & 17.3 & 26.9 & 0.92 & 130 & ... & 2 & ... & ... & ... \\ 
3C~153 & 0.276 & 18.5 & 15.3 & 27.6 & 0.66 & ... & ... & 2 & LEG & 35.74 & ... \\ 
3C~165 & 0.295 & 19.5 & 13.5 & 27.6 & 0.71 & ... & 159 & ... & ... & ... & ... \\ 
3C~166 & 0.245 & 19.5 & 14.7 & 27.4 & 0.90 & ... & 180 & ... & ... & ... & ... \\ 
3C~171 & 0.238 & 18.9 & 19.5 & 27.5 & 0.87 & 30 & 100 & 3 & HEG & 35.70 & 35.90 \\ 
3C~173.1 & 0.292 & 18.9 & 15.4 & 27.6 & 0.88 & 58 & 17 & 2 & LEG & ... & ... \\ 
3C~180 & 0.220 & 19.0 & 15.1 & 27.3 & 0.84 & ... & 7 & ... & ... & ... & ... \\ 
3C~184.1 & 0.118 & 17.0 & 13.0 & 26.7 & 0.68 & 167 & 157 & 2 & WQ & 34.75 & 35.57 \\ 
3C~192 & 0.059 & 15.5 & 21.1 & 26.2 & 0.79 & 200 & ... & 2 & HEG & 34.59 & 34.96 \\ 
3C~196.1 & 0.198 & 17.5 & 18.6 & 27.3 & 1.16 & 4 & 43 & 2 & ... & ... & ... \\ 
3C~197.1 & 0.130 & 16.5 & 8.1 & 26.6 & 0.69 & 14 & 2 & 2 & ... & ... & ... \\ 
3C~198 & 0.081 & 16.8 & 9.7 & 26.2 & 0.69 & 338 & 38 & 2 & ... & ... & ... \\ 
3C~213.1 & 0.194 & 19.0 & 6.6 & 26.9 & 0.55 & 43 & 162 & 2 & ... & ... & ... \\ 
3C~219 & 0.174 & 17.2 & 41.2 & 27.5 & 0.81 & 184 & 40 & 2 & WQ & 34.53 & 35.01 \\ 
3C~223 & 0.136 & 17.1 & 14.7 & 26.9 & 0.74 & 300 & 164 & 2 & WQ & 34.98 & 35.55 \\ 
3C~223.1 & 0.107 & 16.4 & 6.0 & 26.2 & 0.56 & 117 & 15 & 2 & ... & ... & ... \\ 
3C~227 & 0.086 & 16.3 & 30.4 & 26.7 & 0.67 & 246 & 86 & 2 & ... & ... & ... \\ 
3C~234 & 0.184 & 17.3 & 31.4 & 27.5 & 0.86 & 110 & 64 & 2 & WQ & 35.38 & 36.56 \\ 
3C~236 & 0.098 & 16.0 & 14.4 & 26.5 & 0.51 & 2514 & 122 & 3 & LEG & 34.44 & 33.84 \\ 
3C~258 & 0.165 & 19.5 & 9.7 & 26.9 & 1.30 & ... & ... & ... & ... & ... & ... \\ 
3C~264 & 0.020 & 12.7 & 26.0 & 25.4 & 0.75 & 62 & 31 & 1 & FRI & 33.39 & ... \\ 
3C~270 & 0.007 & 10.4 & 51.8 & 24.8 & 0.51 & 407 & 86 & 1 & ... & ... & ... \\ 
3C~272.1 & 0.003 & 8.7 & 19.4 & 23.6 & 0.60 & 178 & 176 & 1 & FRI & ... & ... \\ 
3C~274 & 0.004 & 8.7 & 1050.0 & 25.6 & 0.76 & 933 & 115 & 1 & FRI & ... & ... \\ 
3C~277.3 & 0.085 & 15.9 & 9.0 & 26.2 & 0.58 & 50 & 158 & 2 & ... & ... & ... \\ 
3C~284 & 0.239 & 18.0 & 11.3 & 27.3 & 0.95 & ... & ... & 2 & HEG & ... & 35.59 \\ 
3C~285 & 0.079 & 16.0 & 11.3 & 26.2 & 0.95 & 184 & ... & 2 & HEG & 33.74 & 34.10 \\ 
3C~287.1 & 0.215 & 18.3 & 8.2 & 27.0 & 0.52 & 112 & 91 & 2 & ... & ... & ... \\ 
3C~288 & 0.246 & 18.3 & 18.9 & 27.5 & 0.85 & 16 & 146 & 1 & FRI & ... & ... \\ 
3C~293 & 0.045 & 14.4 & 12.7 & 25.8 & 0.45 & 244 & 92 & 3 & LEG & 34.84 & ... \\ 
3C~296 & 0.023 & 12.2 & 13.0 & 25.2 & 0.67 & ... & ... & 1 & FRI & ... & ... \\ 
3C~300 & 0.270 & 18.0 & 17.9 & 27.6 & 0.75 & ... & ... & 2 & HEG & 35.73 & 35.57 \\ 
3C~303 & 0.141 & 17.0 & 11.2 & 26.8 & 0.76 & 38 & 97 & 2 & WQ & 35.17 & ... \\ 
3C~305 & 0.041 & 13.7 & 15.7 & 25.8 & 0.85 & 13 & 45 & 1 & FRI & 33.41 & ... \\ 
3C~310 & 0.054 & 15.2 & 55.1 & 26.6 & 0.92 & 323 & 165 & 1 & FRI & ... & ... \\ 
3C~314.1 & 0.119 & 17.0 & 10.6 & 26.6 & 0.95 & 201 & 144 & 1 & FRI & ... & ... \\ 
3C~315 & 0.108 & 16.3 & 17.8 & 26.7 & 0.72 & ... & 11 & 1 & FRI & ... & ... \\ 
3C~317 & 0.035 & 13.5 & 49.0 & 26.1 & 1.02 & 59 & 12 & 1 & ... & ... & ... \\ 
3C~319 & 0.192 & 18.5 & 15.3 & 27.2 & 0.90 & 93 & 49 & 2 & LEG & 33.24 & ... \\ 
3C~321 & 0.096 & 16.0 & 13.5 & 26.5 & 0.60 & 309 & 121 & 2 & HEG & 34.59 & 35.52 \\ 
3C~323.1 & 0.264 & 16.7 & 9.7 & 27.3 & 0.65 & ... & ... & ... & ... & ... & ... \\ 
3C~326 & 0.088 & 17.0 & 20.4 & 26.6 & 0.88 & ... & ... & 2 & LEG & 34.52 & 34.01 \\ 
3C~332 & 0.151 & 16.0 & 9.6 & 26.8 & 0.61 & ... & ... & ... & ... & ... & ... \\ 
3C~338 & 0.030 & 12.6 & 46.9 & 26.0 & 1.19 & 110 & 89 & 1 & FRI & 34.08 & ... \\ 
3C~346 & 0.161 & 17.2 & 10.9 & 26.9 & 0.52 & 13 & 71 & 1 & FRI & ... & 34.59 \\ 
3C~348 & 0.154 & 16.9 & 351.0 & 28.4 & 1.00 & 191 & 101 & 2 & ... & ... & ... \\ 
3C~349 & 0.205 & 19.0 & 13.3 & 27.2 & 0.74 & 82 & 142 & 2 & HEG & ... & 34.82 \\ 
3C~353 & 0.030 & 15.4 & 236.0 & 26.7 & 0.71 & 275 & 85 & 2 & ... & ... & ... \\ 
3C~357 & 0.166 & 15.5 & 9.7 & 26.9 & 0.57 & ... & ... & ... & ... & ... & ... \\ 
3C~371 & 0.050 & 14.8 & 3.7 & 25.3 & 0.30 & 277 & 59 & 2 & ... & ... & ... \\ 
3C~379.1 & 0.256 & 18.0 & 7.4 & 27.2 & 0.68 & 76 & 161 & 2 & ... & ... & ... \\ 
3C~381 & 0.160 & 17.5 & 16.6 & 27.1 & 0.81 & 69 & 4 & 2 & HEG & 34.18 & 35.76 \\ 
3C~382 & 0.057 & 14.7 & 19.9 & 26.2 & 0.59 & 179 & 50 & 2 & WQ & 34.01 & 34.88 \\ 
3C~386 & 0.017 & 12.9 & 23.9 & 25.2 & 0.59 & 288 & 17 & 1 & WQ & ... & ... \\ 
3C~388 & 0.090 & 15.7 & 24.6 & 26.7 & 0.70 & 32 & 63 & 2 & HEG & 33.79 & 33.86 \\ 
3C~390.3 & 0.056 & 14.4 & 47.5 & 26.6 & 0.75 & 231 & 145 & 2 & WQ & 34.23 & 35.41 \\ 
3C~401 & 0.201 & 19.1 & 20.9 & 27.4 & 0.71 & 19 & 24 & 2 & LEG & ... & 34.40 \\ 
3C~402 & 0.023 & 14.0 & 10.1 & 25.1 & 0.56 & 528 & 163 & 2 & ... & ... & ... \\ 
3C~403 & 0.059 & 15.4 & 17.8 & 26.2 & 0.45 & 230 & 79 & 2 & ... & ... & ... \\ 
3C~403.1 & 0.055 & 16.0 & 13.5 & 26.0 & 1.12 & ... & ... & ... & ... & ... & ... \\ 
3C~405 & 0.056 & 16.2 & 8700.0 & 28.8 & 0.74 & ... & ... & ... & ... & ... & ... \\ 
3C~410 & 0.248 & 19.5 & 34.6 & 27.8 & 0.56 & ... & ... & ... & ... & ... & ... \\ 
3C~424 & 0.127 & 18.0 & 14.6 & 26.8 & 0.85 & ... & ... & ... & ... & ... & ... \\ 
3C~430 & 0.054 & 15.0 & 33.7 & 26.4 & 0.72 & 99 & 35 & 2 & ... & ... & ... \\ 
3C~433 & 0.101 & 15.5 & 56.2 & 27.2 & 0.75 & 58 & 172 & 2 & HEG & ... & 34.11 \\ 
3C~436 & 0.214 & 18.2 & 17.8 & 27.4 & 0.86 & 105 & 173 & 2 & HEG & ... & 34.92 \\ 
3C~438 & 0.290 & 19.2 & 44.7 & 28.1 & 0.88 & 19 & 136 & 2 & HEG & ... & 34.85 \\ 
3C~442 & 0.026 & 13.7 & 16.1 & 25.4 & 0.96 & ... & ... & ... & ... & ... & ... \\ 
3C~445 & 0.056 & 15.8 & 24.8 & 26.3 & 0.85 & 576 & 171 & 2 & ... & ... & ... \\ 
3C~449 & 0.017 & 13.2 & 11.5 & 24.9 & 0.58 & 1742 & 10 & 1 & FRI & ... & 32.57 \\ 
3C~452 & 0.081 & 16.0 & 54.4 & 26.9 & 0.78 & 277 & 79 & 2 & HEG & 34.72 & ... \\ 
3C~459 & 0.219 & 17.6 & 25.6 & 27.6 & 0.74 & ... & ... & ... & ... & ... & ... \\ 
3C~465 & 0.029 & 13.2 & 37.8 & 25.9 & 0.75 & 375 & 122 & 1 & FRI & ... & ... \\ 
  \enddata
  \tablecomments{Main radio and optical properties for each source:
    redshift; 
    V-band magnitude; 
    radio flux density in Janskys at 178~MHz; 
    radio  power at  178~MHz  in W~Hz$^{-1}$; 
    radio spectral index; 
    radio source largest angular size; 
    radio structure position angle; 
    Faranoff-Riley class;
    Ionisation Class;
    [OII]~3727 emission line luminosity in W;
    [OIII]~5007 emission line luminosity in W.}
  \tablerefs{$^{a}$~\citet{spinrad+85} -- updated values were taken from the 
    NASA Extragalactic Database (NED);
    $^{b}$~\citet{dekoff+96} and references therein; 
    $^{c}$~\citet{martel+99} and references therein;
    $^{d}$~\citet{jacksonrawlings97}.}
\end{deluxetable}


==> tab4.tex <==
% Table 4: ELLIPSE RESULTS
\begin{deluxetable}{llrrllrrrr}
  \tabletypesize{\tiny}
  \tablecolumns{10}
  \tablewidth{0pc} 
  \renewcommand{\arraystretch}{.6}
  \tablecaption{\label{tab-ellipse} Ellipse and 1-D \sersic model fits}
  \tablehead{
    \colhead{Source} & 
    \colhead{$(1-b/a)_{\mathrm med}$} & 
    \colhead{$\theta_{\mathrm med}$} &
    \colhead{$a_3/a_{\mathrm min}$} &
    \colhead{$a_3/a_{\mathrm max}$} &
    \colhead{$a_4/a_{\mathrm min}$} & 
    \colhead{$a_4/a_{\mathrm max}$} &
    \colhead{$r_e$/kpc} & 
    \colhead{$\langle\mu\rangle_e$} & 
    \colhead{$n$}}
  \startdata
  %    \input{/Users/floyd/3C/Work/idl/ellipse}
3C~15 & 0.06 & 21.32 & -0.08 & 0.02 & -0.04 & 0.02 &$4.96\pm 0.45$&$19.76\pm 0.13$&$4.17\pm 0.08$\\ 
3C~17 & 0.17 & 21.32 & -0.17 & 0.06 & -0.08 & 0.14 &$5.84\pm 1.53$&$20.69\pm 0.52$&$10.00\pm 0.00$\\ 
3C~20 & 0.10 & -63.77 & -0.06 & 0.10 & -0.03 & 0.20 &$2.72\pm 1.45$&$19.17\pm 1.05$&$3.23\pm 0.54$\\ 
3C~28 & 0.18 & -26.43 & -0.03 & 0.11 & -0.04 & 0.03 &$6.74\pm 0.63$&$20.26\pm 0.11$&$2.01\pm 0.08$\\ 
3C~29 & 0.03 & -76.28 & -0.05 & 0.02 & -0.05 & 0.03 &$4.44\pm 0.15$&$19.05\pm 0.02$&$1.50\pm 0.02$\\ 
3C~31 & 0.12 & -32.23 & -0.02 & 0.08 & -0.03 & 0.01 &$1.46\pm 0.05$&$17.20\pm 0.02$&$1.43\pm 0.02$\\ 
3C~33 & 0.07 & -43.84 & -0.09 & 0.01 & -0.04 & 0.06 &$2.75\pm 0.21$&$18.97\pm 0.11$&$3.19\pm 0.07$\\ 
3C~33.1 & 0.06 & 13.96 & -0.02 & 0.03 & -0.05 & 0.02 &$2.19\pm 0.65$&$18.66\pm 0.65$&$4.49\pm 0.33$\\ 
3C~35 & 0.23 & -65.28 & -0.18 & 0.02 & -0.07 & 0.03 &$4.59\pm 0.67$&$19.89\pm 0.20$&$3.60\pm 0.14$\\ 
3C~52 & 0.31 & 10.96 & -0.03 & 0.06 & -0.02 & 0.08 &$3.55\pm 0.36$&$18.74\pm 0.18$&$1.73\pm 0.09$\\ 
3C~61.1 & 0.09 & 0.95 & -0.17 & 0.22 & -0.07 & 0.08 &$1.87\pm 0.16$&$19.65\pm 0.20$&$2.07\pm 0.11$\\ 
3C~66B & 0.06 & -50.32 & -0.08 & 0.04 & -0.03 & 0.06 &$2.42\pm 0.15$&$18.42\pm 0.04$&$1.97\pm 0.05$\\ 
3C~71 & 0.18 & 36.54 & -0.04 & 0.03 & -0.06 & 0.02 &$2.21\pm 0.51$&$19.51\pm 0.35$&$10.00\pm 0.00$\\ 
3C~75N & 0.19 & -80.47 & -0.01 & 0.05 & -0.02 & 0.04 &$1.64\pm 0.22$&$17.75\pm 0.16$&$3.09\pm 0.12$\\ 
3C~76.1 & 0.14 & -47.79 & -0.02 & 0.04 & -0.05 & 0.02 &$1.12\pm 0.07$&$17.95\pm 0.09$&$2.26\pm 0.06$\\ 
3C~79 & 0.18 & 8.69 & -0.07 & 0.06 & -0.08 & 0.03 &$3.31\pm 0.99$&$19.20\pm 0.60$&$3.23\pm 0.30$\\ 
3C~83.1 & 0.23 & -9.56 & -0.14 & 0.06 & -0.05 & 0.04 &$1.84\pm 0.14$&$17.33\pm 0.06$&$1.60\pm 0.06$\\ 
3C~84 & 0.19 & -64.36 & -0.06 & 0.04 & -0.05 & 0.10 &$6.20\pm 20.65$&$46.96\pm 4.37$&$6.27\pm 3.14$\\ 
3C~88 & 0.15 & -30.08 & -0.02 & 0.02 & -0.06 & 0.04 &$3.02\pm 0.31$&$19.51\pm 0.09$&$2.40\pm 0.09$\\ 
3C~98 & 0.14 & 52.77 & -0.01 & 0.02 & -0.01 & 0.02 &$1.93\pm 0.24$&$18.71\pm 0.18$&$3.75\pm 0.11$\\ 
3C~105 & 0.22 & 50.41 & -0.06 & 0.01 & -0.05 & 0.26 &$1.64\pm 0.28$&$18.68\pm 0.31$&$2.78\pm 0.16$\\ 
3C~111 & 0.16 & 22.21 & -0.08 & 0.04 & -0.05 & 0.07 &$0.20\pm 0.03$&$12.95\pm 0.32$&$10.00\pm 0.00$\\ 
3C~123 & 0.06 & -72.85 & -0.05 & 0.04 & -0.06 & 0.03 &$10.47\pm 1.55$&$20.79\pm 0.20$&$3.16\pm 0.14$\\ 
3C~129 & 0.13 & -46.09 & -0.02 & 0.03 & -0.05 & 0.07 &$1.97\pm 0.06$&$18.04\pm 0.02$&$1.63\pm 0.02$\\ 
3C~129.1 & 0.05 & 8.75 & -0.02 & 0.05 & -0.04 & 0.01 &$2.55\pm 0.07$&$18.13\pm 0.01$&$1.38\pm 0.02$\\ 
3C~130 & 0.19 & -65.59 & -0.09 & 0.08 & -0.02 & 0.04 &$6.71\pm 0.47$&$17.78\pm 0.07$&$2.32\pm 0.06$\\ 
3C~132 & 0.17 & 19.05 & 0.00 & 0.01 & -0.02 & 0.01 &$6.42\pm 1.20$&$19.94\pm 0.31$&$3.49\pm 0.19$\\ 
3C~133 & 0.07 & -16.58 & -0.12 & 0.06 & -0.11 & 0.04 &$1.63\pm 1.38$&$17.61\pm 2.04$&$6.53\pm 0.92$\\ 
3C~135 & 0.15 & -48.30 & -0.06 & 0.09 & -0.06 & 0.03 &$4.81\pm 3.71$&$20.58\pm 1.40$&$5.89\pm 0.79$\\ 
3C~153 & 0.10 & -69.56 & -0.06 & 0.01 & -0.06 & 0.01 &$4.94\pm 1.07$&$19.88\pm 0.41$&$3.42\pm 0.21$\\ 
3C~165 & 0.15 & 0.27 & -0.01 & 0.12 & -0.05 & 0.04 &$3.86\pm 0.63$&$19.42\pm 0.31$&$0.95\pm 0.11$\\ 
3C~166 & 0.09 & -51.90 & -0.05 & 0.69 & -0.19 & 0.04 &$56.94\pm 13.20$&$24.96\pm 0.37$&$10.00\pm 0.00$\\ 
3C~171 & 0.07 & -54.58 & -0.14 & 0.38 & -0.05 & 0.27 &$2.04\pm 1.09$&$18.75\pm 1.24$&$10.00\pm 0.00$\\ 
3C~173.1 & 0.25 & 13.00 & -0.11 & 0.04 & -0.09 & 0.01 &$2.83\pm 0.18$&$18.46\pm 0.14$&$1.76\pm 0.08$\\ 
3C~180 & 0.40 & 29.39 & -0.05 & 0.04 & -0.02 & 0.03 &$6.44\pm 1.12$&$20.60\pm 0.26$&$2.77\pm 0.18$\\ 
3C~184.1 & 0.20 & 44.78 & -0.10 & 0.07 & -0.08 & 0.10 &$0.97\pm 0.22$&$17.41\pm 0.56$&$3.74\pm 0.25$\\ 
3C~192 & 0.02 & 18.34 & -0.17 & 0.09 & -0.03 & 0.07 &$2.03\pm 0.13$&$18.41\pm 0.09$&$2.65\pm 0.06$\\ 
3C~196.1 & 0.29 & 53.10 & -0.01 & 0.08 & -0.11 & 0.01 &$14.43\pm 0.89$&$21.42\pm 0.06$&$2.54\pm 0.06$\\ 
3C~197.1 & 0.05 & -13.38 & -0.03 & 0.02 & -0.02 & 0.06 &$3.27\pm 0.41$&$19.55\pm 0.22$&$3.55\pm 0.13$\\ 
3C~198 & 0.09 & 63.47 & -0.22 & 0.06 & -0.03 & 0.11 &$1.59\pm 0.30$&$19.06\pm 0.36$&$3.80\pm 0.19$\\ 
3C~213.1 & 0.31 & -61.99 & -0.02 & 0.03 & -0.01 & 0.07 &$2.10\pm 0.18$&$19.00\pm 0.19$&$2.50\pm 0.10$\\ 
3C~219 & 0.19 & -56.55 & -0.05 & 0.04 & -0.02 & 0.03 &$4.89\pm 0.84$&$19.92\pm 0.31$&$4.51\pm 0.18$\\ 
3C~223 & 0.14 & 72.19 & -0.08 & 0.11 & -0.14 & 0.11 &$4.54\pm 0.75$&$20.12\pm 0.27$&$3.66\pm 0.17$\\ 
3C~223.1 & 0.21 & 37.50 & -0.11 & 0.07 & -0.01 & 0.05 &$7.94\pm 9.49$&$21.08\pm 2.16$&$8.90\pm 1.24$\\ 
3C~227 & 0.10 & -2.33 & -0.04 & 0.09 & -0.08 & 0.08 &$0.32\pm 0.03$&$14.62\pm 0.26$&$10.00\pm 0.00$\\ 
3C~234 & 0.11 & 38.66 & -0.13 & 0.04 & -0.06 & 0.06 &$0.35\pm 0.07$&$14.05\pm 0.55$&$10.00\pm 0.00$\\ 
3C~236 & 0.31 & 48.71 & -0.07 & 0.02 & -0.03 & 0.03 &$3.18\pm 0.39$&$19.25\pm 0.20$&$3.65\pm 0.12$\\ 
3C~258 & 0.24 & -27.25 & -0.38 & 0.02 & -0.05 & 0.09 &$6.05\pm 3.09$&$24.05\pm 0.95$&$10.00\pm 0.00$\\ 
3C~264 & 0.03 & 19.06 & -0.08 & 0.03 & -0.01 & 0.06 &$1.05\pm 0.05$&$17.29\pm 0.04$&$1.28\pm 0.03$\\ 
3C~270 & 0.27 & -22.53 & -0.03 & 0.03 & -0.03 & 0.03 &$0.88\pm 0.10$&$17.02\pm 0.05$&$1.40\pm 0.07$\\ 
3C~272.1 & 0.17 & -48.96 & -0.01 & 0.02 & -0.03 & 0.01 &$0.33\pm 0.01$&$16.23\pm 0.02$&$1.26\pm 0.02$\\ 
3C~274 & 0.02 & -30.24 & -0.05 & 0.03 & -0.02 & 0.07 &$63004.1\pm 26195.0$&$31.14\pm 0.24$&$10.00\pm 0.00$\\ 
3C~277.3 & 0.06 & -25.19 & -0.08 & 0.06 & -0.09 & 0.06 &$3.01\pm 0.15$&$19.02\pm 0.06$&$1.99\pm 0.04$\\ 
3C~284 & 0.16 & 40.70 & -0.04 & 0.08 & -0.02 & 0.07 &$4.34\pm 1.83$&$19.54\pm 0.77$&$2.97\pm 0.40$\\ 
3C~285 & 0.29 & -53.56 & -0.02 & 0.04 & -0.03 & 0.06 &$3.08\pm 0.12$&$19.44\pm 0.05$&$2.33\pm 0.04$\\ 
3C~287.1 & 0.07 & 30.58 & -0.63 & 0.06 & -0.07 & 0.06 &$1.94\pm 0.27$&$18.22\pm 0.29$&$10.00\pm 0.00$\\ 
3C~288 & 0.05 & -43.35 & -0.09 & 0.10 & -0.06 & 0.06 &$7.82\pm 0.14$&$19.72\pm 0.01$&$1.29\pm 0.01$\\ 
3C~293 & 0.38 & 57.63 & -0.03 & 0.06 & -0.03 & 0.04 &$6.97\pm 1.04$&$20.70\pm 0.16$&$3.46\pm 0.13$\\ 
3C~296 & 0.25 & -34.23 & -0.01 & 0.01 & -0.05 & 0.02 &$2.76\pm 0.37$&$17.97\pm 0.10$&$2.03\pm 0.10$\\ 
3C~300 & 0.27 & -52.95 & -0.04 & 0.14 & -0.03 & 0.19 &$1.91\pm 0.89$&$18.99\pm 1.20$&$2.46\pm 0.47$\\ 
3C~303 & 0.09 & -13.25 & -0.01 & 0.04 & -0.05 & 0.06 &$4.04\pm 2.08$&$19.65\pm 1.01$&$7.78\pm 0.53$\\ 
3C~305 & 0.19 & 69.16 & -0.02 & 0.01 & -0.02 & 0.01 &$14.65\pm 6.80$&$13.08\pm 0.66$&$7.52\pm 0.46$\\ 
3C~310 & 0.29 & 84.60 & -0.02 & 0.01 & -0.02 & 0.02 &$2.83\pm 0.22$&$19.48\pm 0.08$&$2.25\pm 0.07$\\ 
3C~314.1 & 0.33 & 71.30 & -0.01 & 0.20 & -0.15 & 0.10 &$2.04\pm 0.21$&$19.37\pm 0.19$&$2.58\pm 0.10$\\ 
3C~315 & 0.41 & 35.08 & -0.01 & 0.05 & -0.04 & 0.02 &$1.66\pm 0.43$&$18.71\pm 0.53$&$3.34\pm 0.27$\\ 
3C~317 & 0.09 & 33.09 & -0.06 & 0.03 & -0.04 & 0.03 &$9.20\pm 1.51$&$21.21\pm 0.14$&$3.18\pm 0.14$\\ 
3C~319 & 0.12 & -36.22 & -0.13 & 0.01 & -0.02 & 0.07 &$5.28\pm 4.33$&$21.09\pm 1.58$&$6.10\pm 0.91$\\ 
3C~321 & 0.12 & 70.57 & -0.02 & 0.02 & -0.02 & 0.05 &$3.47\pm 0.33$&$18.91\pm 0.13$&$2.31\pm 0.07$\\ 
3C~323.1 & 0.08 & 59.14 & -0.09 & 0.05 & -0.17 & 0.05 &$0.18\pm 0.04$&$11.37\pm 0.62$&$10.00\pm 0.00$\\ 
3C~326 & 0.31 & -76.53 & -0.08 & 0.13 & -0.01 & 0.06 &$1.39\pm 0.45$&$18.45\pm 0.66$&$3.84\pm 0.31$\\ 
3C~332 & 0.08 & -48.25 & -0.03 & 0.14 & -0.08 & 0.10 &$1.12\pm 0.89$&$16.76\pm 1.95$&$4.47\pm 0.79$\\ 
3C~338 & 0.12 & 33.10 & -0.04 & 0.03 & -0.02 & 0.03 &$8.71\pm 0.72$&$10.23\pm 0.02$&$1.41\pm 0.05$\\ 
3C~346 & 0.16 & -53.43 & -0.04 & 0.12 & -0.10 & 0.03 &$2.55\pm 1.51$&$19.19\pm 1.21$&$3.84\pm 0.63$\\ 
3C~348 & 0.24 & -61.47 & -0.06 & 0.07 & -0.05 & 0.03 &$6.43\pm 0.11$&$20.09\pm 0.01$&$0.91\pm 0.01$\\ 
3C~349 & 0.31 & 21.82 & -0.01 & 0.02 & -0.11 & 0.00 &$2.49\pm 1.96$&$19.61\pm 1.72$&$6.15\pm 0.86$\\ 
3C~353 & 0.04 & 75.59 & -0.04 & 0.04 & -0.04 & 0.02 &$1.89\pm 0.22$&$18.47\pm 0.14$&$2.84\pm 0.10$\\ 
3C~357 & 0.30 & 79.66 & -0.02 & 0.08 & -0.05 & 0.10 &$5.22\pm 1.33$&$19.81\pm 0.45$&$4.43\pm 0.24$\\ 
3C~371 & 0.08 & 44.98 & -0.06 & 0.04 & -0.08 & 0.04 &$0.33\pm 0.06$&$14.12\pm 0.38$&$10.00\pm 0.00$\\ 
3C~379.1 & 0.08 & -46.38 & -0.01 & 0.07 & -0.01 & 0.05 &$5.06\pm 0.54$&$19.33\pm 0.17$&$1.53\pm 0.08$\\ 
3C~381 & 0.15 & 62.19 & -0.07 & 0.72 & -0.65 & 0.03 &$2.62\pm 0.49$&$19.00\pm 0.36$&$3.35\pm 0.18$\\ 
3C~382 & 0.17 & 77.69 & -0.04 & 0.07 & -0.12 & 0.06 &$0.53\pm 0.09$&$14.71\pm 0.35$&$10.00\pm 0.00$\\ 
3C~386 & 0.07 & -53.79 & -0.03 & 0.04 & -0.11 & 0.09 &$13.89\pm 2.31$&$22.45\pm 0.24$&$10.00\pm 0.00$\\ 
3C~388 & 0.15 & 39.34 & -0.06 & 0.03 & -0.02 & 0.05 &$6.06\pm 0.18$&$19.35\pm 0.02$&$1.56\pm 0.02$\\ 
3C~390.3 & 0.12 & 23.96 & -0.04 & 0.07 & -0.08 & 0.06 &$0.47\pm 0.04$&$15.32\pm 0.21$&$10.00\pm 0.00$\\ 
3C~401 & 0.10 & -78.88 & -0.07 & 0.05 & -0.24 & 0.08 &$9.91\pm 0.99$&$21.27\pm 0.12$&$2.61\pm 0.09$\\ 
3C~402 & 0.17 & 35.86 & -0.04 & 0.01 & -0.06 & 0.01 &$1.45\pm 0.10$&$17.87\pm 0.07$&$2.27\pm 0.06$\\ 
3C~403 & 0.21 & 35.26 & -0.07 & 0.03 & -0.02 & 0.03 &$4.89\pm 0.30$&$19.62\pm 0.08$&$3.78\pm 0.06$\\ 
3C~403.1 & 0.14 & -27.59 & -0.09 & 0.04 & -0.02 & 0.08 &$1.28\pm 0.13$&$17.97\pm 0.18$&$3.13\pm 0.09$\\ 
3C~405 & 0.23 & -15.10 & -0.07 & 0.10 & -0.05 & 0.06 &$2.82\pm 0.25$&$18.96\pm 0.04$&$0.79\pm 0.04$\\ 
3C~410 & 0.11 & 48.47 & -0.06 & 0.08 & -0.10 & 0.17 &$1.35\pm 1.94$&$41.84\pm 3.61$&$5.61\pm 1.46$\\ 
3C~424 & 0.05 & 37.18 & -0.02 & 0.03 & -0.11 & 0.10 &$5.38\pm 1.04$&$21.10\pm 0.32$&$4.70\pm 0.20$\\ 
3C~430 & 0.30 & -73.67 & -0.05 & 0.06 & -0.02 & 0.02 &$1.92\pm 0.25$&$18.09\pm 0.20$&$2.78\pm 0.12$\\ 
3C~433 & 0.30 & -28.14 & -0.07 & 0.04 & -0.02 & 0.03 &$23.85\pm 24.40$&$22.89\pm 1.66$&$9.61\pm 1.06$\\ 
3C~436 & 0.18 & 16.22 & -0.06 & 0.07 & -0.09 & 0.01 &$4.67\pm 0.80$&$19.66\pm 0.28$&$2.70\pm 0.16$\\ 
3C~438 & 0.04 & -7.92 & -0.02 & 0.56 & -0.37 & 0.06 &$5.55\pm 0.22$&$19.46\pm 0.06$&$1.88\pm 0.04$\\ 
3C~442 & 0.13 & -47.05 & -0.02 & 0.07 & -0.04 & 0.03 &$1.44\pm 0.04$&$43.60\pm 0.02$&$1.17\pm 0.02$\\ 
3C~445 & 0.10 & 57.80 & -0.25 & 0.09 & -0.06 & 0.14 &$0.12\pm 0.01$&$12.43\pm 0.29$&$10.00\pm 0.00$\\ 
3C~449 & 0.15 & -17.18 & -0.09 & 0.00 & -0.01 & 0.02 &$0.97\pm 0.02$&$17.29\pm 0.02$&$1.38\pm 0.01$\\ 
3C~452 & 0.26 & -75.69 & -0.04 & 0.09 & -0.02 & 0.01 &$2.61\pm 0.24$&$18.83\pm 0.14$&$2.94\pm 0.09$\\ 
3C~459 & 0.06 & 24.45 & -0.09 & 0.04 & -0.13 & 0.13 &$2.22\pm 0.26$&$18.26\pm 0.26$&$10.00\pm 0.00$\\ 
3C~465 & 0.09 & 28.95 & -0.09 & 0.04 & -0.04 & 0.04 &$2.39\pm 0.19$&$17.85\pm 0.06$&$1.66\pm 0.06$\\ 
%   3C~15 & 0.06 & 21.32 & -0.08 & 0.02 & -0.04 & 0.02 & 4.96 & 19.76 & 4.17 \\ 
%   3C~17 & 0.17 & 21.32 & -0.17 & 0.06 & -0.08 & 0.14 & 5.84 & 20.69 & 10.00 \\ 
%   3C~20 & 0.10 & -63.77 & -0.06 & 0.10 & -0.03 & 0.20 & 2.72 & 19.17 & 3.23 \\ 
%   3C~28 & 0.18 & -26.43 & -0.03 & 0.11 & -0.04 & 0.03 & 6.74 & 20.26 & 2.01 \\ 
%   3C~29 & 0.03 & -76.28 & -0.05 & 0.02 & -0.05 & 0.03 & 4.44 & 19.05 & 1.50 \\ 
%   3C~31 & 0.12 & -32.23 & -0.02 & 0.08 & -0.03 & 0.01 & 1.46 & 17.20 & 1.43 \\ 
%   3C~33 & 0.07 & -43.84 & -0.09 & 0.01 & -0.04 & 0.06 & 2.75 & 18.97 & 3.19 \\ 
%   3C~33.1 & 0.06 & 13.96 & -0.02 & 0.03 & -0.05 & 0.02 & 2.19 & 18.66 & 4.49 \\ 
%   3C~35 & 0.23 & -65.28 & -0.18 & 0.02 & -0.07 & 0.03 & 4.59 & 19.89 & 3.60 \\ 
%   3C~52 & 0.31 & 10.96 & -0.03 & 0.06 & -0.02 & 0.08 & 3.55 & 18.74 & 1.73 \\ 
%   3C~61.1 & 0.09 & 0.95 & -0.17 & 0.22 & -0.07 & 0.08 & 1.87 & 19.65 & 2.07 \\ 
%   3C~66B & 0.06 & -50.32 & -0.08 & 0.04 & -0.03 & 0.06 & 2.42 & 18.42 & 1.97 \\ 
%   3C~71 & 0.18 & 36.54 & -0.04 & 0.03 & -0.06 & 0.02 & ... & ... & 10.00 \\ 
%   3C~75N & 0.19 & -80.47 & -0.01 & 0.05 & -0.02 & 0.04 & 1.64 & 17.75 & 3.09 \\ 
%   3C~76.1 & 0.14 & -47.79 & -0.02 & 0.04 & -0.05 & 0.02 & 1.12 & 17.95 & 2.26 \\ 
%   3C~79 & 0.18 & 8.69 & -0.07 & 0.06 & -0.08 & 0.03 & 3.31 & 19.20 & 3.23 \\ 
%   3C~83.1 & 0.23 & -9.56 & -0.14 & 0.06 & -0.05 & 0.04 & 1.84 & 17.33 & 1.60 \\ 
%   3C~84 & 0.19 & -64.36 & -0.06 & 0.04 & -0.05 & 0.10 & 6.20 & 46.96 & 6.27 \\ 
%   3C~88 & 0.15 & -30.08 & -0.02 & 0.02 & -0.06 & 0.04 & 3.02 & 19.51 & 2.40 \\ 
%   3C~98 & 0.14 & 52.77 & -0.01 & 0.02 & -0.01 & 0.02 & 1.93 & 18.71 & 3.75 \\ 
%   3C~105 & 0.22 & 50.41 & -0.06 & 0.01 & -0.05 & 0.26 & 1.64 & 18.68 & 2.78 \\ 
%   3C~111 & 0.16 & 22.21 & -0.08 & 0.04 & -0.05 & 0.07 & 0.20 & 12.95 & 10.00 \\ 
%   3C~123 & 0.06 & -72.85 & -0.05 & 0.04 & -0.06 & 0.03 & 10.47 & 20.79 & 3.16 \\ 
%   3C~129 & 0.13 & -46.09 & -0.02 & 0.03 & -0.05 & 0.07 & 1.97 & 18.04 & 1.63 \\ 
%   3C~129.1 & 0.05 & 8.75 & -0.02 & 0.05 & -0.04 & 0.01 & 2.55 & 18.13 & 1.38 \\ 
%   3C~130 & 0.19 & -65.59 & -0.09 & 0.08 & -0.02 & 0.04 & 6.71 & 17.78 & 2.32 \\ 
%   3C~132 & 0.17 & 19.05 & 0.00 & 0.01 & -0.02 & 0.01 & 6.42 & 19.94 & 3.49 \\ 
%   3C~133 & 0.07 & -16.58 & -0.12 & 0.06 & -0.11 & 0.04 & 1.63 & 17.61 & 6.53 \\ 
%   3C~135 & 0.15 & -48.30 & -0.06 & 0.09 & -0.06 & 0.03 & 4.81 & 20.58 & 5.89 \\ 
%   3C~153 & 0.10 & -69.56 & -0.06 & 0.01 & -0.06 & 0.01 & 4.94 & 19.88 & 3.42 \\ 
%   3C~165 & 0.15 & 0.27 & -0.01 & 0.12 & -0.05 & 0.04 & 3.86 & 19.42 & 0.95 \\ 
%   3C~166 & 0.09 & -51.90 & -0.05 & 0.69 & -0.19 & 0.04 & 56.94 & 24.96 & 10.00 \\ 
%   3C~171 & 0.07 & -54.58 & -0.14 & 0.38 & -0.05 & 0.27 & 2.04 & 18.75 & 10.00 \\ 
%   3C~173.1 & 0.25 & 13.00 & -0.11 & 0.04 & -0.09 & 0.01 & 2.83 & 18.46 & 1.76 \\ 
%   3C~180 & 0.40 & 29.39 & -0.05 & 0.04 & -0.02 & 0.03 & 6.44 & 20.60 & 2.77 \\ 
%   3C~184.1 & 0.20 & 44.78 & -0.10 & 0.07 & -0.08 & 0.10 & 0.97 & 17.41 & 3.74 \\ 
%   3C~192 & 0.02 & 18.34 & -0.17 & 0.09 & -0.03 & 0.07 & 2.03 & 18.41 & 2.65 \\ 
%   3C~196.1 & 0.29 & 53.10 & -0.01 & 0.08 & -0.11 & 0.01 & 14.43 & 21.42 & 2.54 \\ 
%   3C~197.1 & 0.05 & -13.38 & -0.03 & 0.02 & -0.02 & 0.06 & 3.27 & 19.55 & 3.55 \\ 
%   3C~198 & 0.09 & 63.47 & -0.22 & 0.06 & -0.03 & 0.11 & 1.59 & 19.06 & 3.80 \\ 
%   3C~213.1 & 0.31 & -61.99 & -0.02 & 0.03 & -0.01 & 0.07 & 2.10 & 19.00 & 2.50 \\ 
%   3C~219 & 0.19 & -56.55 & -0.05 & 0.04 & -0.02 & 0.03 & 4.89 & 19.92 & 4.51 \\ 
%   3C~223 & 0.14 & 72.19 & -0.08 & 0.11 & -0.14 & 0.11 & 4.54 & 20.12 & 3.66 \\ 
%   3C~223.1 & 0.21 & 37.50 & -0.11 & 0.07 & -0.01 & 0.05 & 7.94 & 21.08 & 8.90 \\ 
%   3C~227 & 0.10 & -2.33 & -0.04 & 0.09 & -0.08 & 0.08 & 0.32 & 14.62 & 10.00 \\ 
%   3C~234 & 0.11 & 38.66 & -0.13 & 0.04 & -0.06 & 0.06 & 0.35 & 14.05 & 10.00 \\ 
%   3C~236 & 0.31 & 48.71 & -0.07 & 0.02 & -0.03 & 0.03 & 3.18 & 19.25 & 3.65 \\ 
%   3C~258 & 0.24 & -27.25 & -0.38 & 0.02 & -0.05 & 0.09 & 6.05 & 24.05 & 10.00 \\ 
%   3C~264 & 0.03 & 19.06 & -0.08 & 0.03 & -0.01 & 0.06 & 1.05 & 17.29 & 1.28 \\ 
%   3C~270 & 0.27 & -22.53 & -0.03 & 0.03 & -0.03 & 0.03 & 0.88 & 17.02 & 1.40 \\ 
%   3C~272.1 & 0.17 & -48.96 & -0.01 & 0.02 & -0.03 & 0.01 & 0.33 & 16.23 & 1.26 \\ 
%   3C~274 & 0.02 & -30.24 & -0.05 & 0.03 & -0.02 & 0.07 & ... & ... & 10.00 \\ 
%   3C~277.3 & 0.06 & -25.19 & -0.08 & 0.06 & -0.09 & 0.06 & 3.01 & 19.02 & 1.99 \\ 
%   3C~284 & 0.16 & 40.70 & -0.04 & 0.08 & -0.02 & 0.07 & 4.34 & 19.54 & 2.97 \\ 
%   3C~285 & 0.29 & -53.56 & -0.02 & 0.04 & -0.03 & 0.06 & 3.08 & 19.44 & 2.33 \\ 
%   3C~287.1 & 0.07 & 30.58 & -0.63 & 0.06 & -0.07 & 0.06 & 1.94 & 18.22 & 10.00 \\ 
%   3C~288 & 0.05 & -43.35 & -0.09 & 0.10 & -0.06 & 0.06 & 7.82 & 19.72 & 1.29 \\ 
%   3C~293 & 0.38 & 57.63 & -0.03 & 0.06 & -0.03 & 0.04 & 6.97 & 20.70 & 3.46 \\ 
%   3C~296 & 0.25 & -34.23 & -0.01 & 0.01 & -0.05 & 0.02 & 2.76 & 17.97 & 2.03 \\ 
%   3C~300 & 0.27 & -52.95 & -0.04 & 0.14 & -0.03 & 0.19 & 1.91 & 18.99 & 2.46 \\ 
%   3C~303 & 0.09 & -13.25 & -0.01 & 0.04 & -0.05 & 0.06 & 4.03 & 19.65 & 7.78 \\ 
%   3C~305 & 0.19 & 69.16 & -0.02 & 0.01 & -0.02 & 0.01 & 14.65 & 13.08 & 7.52 \\ 
%   3C~310 & 0.29 & 84.60 & -0.02 & 0.01 & -0.02 & 0.02 & 2.83 & 19.48 & 2.25 \\ 
%   3C~314.1 & 0.33 & 71.30 & -0.01 & 0.20 & -0.15 & 0.10 & 2.04 & 19.37 & 2.58 \\ 
%   3C~315 & 0.41 & 35.08 & -0.01 & 0.05 & -0.04 & 0.02 & 1.66 & 18.71 & 3.34 \\ 
%   3C~317 & 0.09 & 33.09 & -0.06 & 0.03 & -0.04 & 0.03 & 9.20 & 21.21 & 3.18 \\ 
%   3C~319 & 0.12 & -36.22 & -0.13 & 0.01 & -0.02 & 0.07 & 5.28 & 21.09 & 6.10 \\ 
%   3C~321 & 0.12 & 70.57 & -0.02 & 0.02 & -0.02 & 0.05 & 3.47 & 18.91 & 2.31 \\ 
%   3C~323.1 & 0.08 & 59.14 & -0.09 & 0.05 & -0.17 & 0.05 & 0.18 & 11.37 & 10.00 \\ 
%   3C~326 & 0.31 & -76.53 & -0.08 & 0.13 & -0.01 & 0.06 & 1.39 & 18.45 & 3.84 \\ 
%   3C~332 & 0.08 & -48.25 & -0.03 & 0.14 & -0.08 & 0.10 & 1.12 & 16.76 & 4.47 \\ 
%   3C~338 & 0.12 & 33.10 & -0.04 & 0.03 & -0.02 & 0.03 & 8.71 & 10.23 & 1.41 \\ 
%   3C~346 & 0.16 & -53.43 & -0.04 & 0.12 & -0.10 & 0.03 & 2.55 & 19.19 & 3.84 \\ 
%   3C~348 & 0.24 & -61.47 & -0.06 & 0.07 & -0.05 & 0.03 & 6.43 & 20.09 & 0.91 \\ 
%   3C~349 & 0.31 & 21.82 & -0.01 & 0.02 & -0.11 & 0.00 & 2.49 & 19.61 & 6.15 \\ 
%   3C~353 & 0.04 & 75.59 & -0.04 & 0.04 & -0.04 & 0.02 & 1.89 & 18.47 & 2.84 \\ 
%   3C~357 & 0.30 & 79.66 & -0.02 & 0.08 & -0.05 & 0.10 & 5.22 & 19.81 & 4.43 \\ 
%   3C~371 & 0.08 & 44.98 & -0.06 & 0.04 & -0.08 & 0.04 & 0.33 & 14.12 & 10.00 \\ 
%   3C~379.1 & 0.08 & -46.38 & -0.01 & 0.07 & -0.01 & 0.05 & 5.06 & 19.33 & 1.53 \\ 
%   3C~381 & 0.15 & 62.19 & -0.07 & 0.72 & -0.65 & 0.03 & 2.62 & 19.00 & 3.35 \\ 
%   3C~382 & 0.17 & 77.69 & -0.04 & 0.07 & -0.12 & 0.06 & 0.53 & 14.71 & 10.00 \\ 
%   3C~386 & 0.07 & -53.79 & -0.03 & 0.04 & -0.11 & 0.09 & 13.89 & 22.45 & 10.00 \\ 
%   3C~388 & 0.15 & 39.34 & -0.06 & 0.03 & -0.02 & 0.05 & 6.06 & 19.35 & 1.56 \\ 
%   3C~390.3 & 0.12 & 23.96 & -0.04 & 0.07 & -0.08 & 0.06 & 0.47 & 15.32 & 10.00 \\ 
%   3C~401 & 0.10 & -78.88 & -0.07 & 0.05 & -0.24 & 0.08 & 9.91 & 21.27 & 2.61 \\ 
%   3C~402 & 0.17 & 35.86 & -0.04 & 0.01 & -0.06 & 0.01 & 1.45 & 17.87 & 2.27 \\ 
%   3C~403 & 0.21 & 35.26 & -0.07 & 0.03 & -0.02 & 0.03 & 4.89 & 19.62 & 3.78 \\ 
%   3C~403.1 & 0.14 & -27.59 & -0.09 & 0.04 & -0.02 & 0.08 & 1.28 & 17.97 & 3.13 \\ 
%   3C~405 & 0.23 & -15.10 & -0.07 & 0.10 & -0.05 & 0.06 & 2.82 & 18.96 & 0.79 \\ 
%   3C~410 & 0.11 & 48.47 & -0.06 & 0.08 & -0.10 & 0.17 & 1.35 & 41.84 & 5.61 \\ 
%   3C~424 & 0.05 & 37.18 & -0.02 & 0.03 & -0.11 & 0.10 & 5.38 & 21.10 & 4.70 \\ 
%   3C~430 & 0.30 & -73.67 & -0.05 & 0.06 & -0.02 & 0.02 & 1.92 & 18.09 & 2.78 \\ 
%   3C~433 & 0.30 & -28.14 & -0.07 & 0.04 & -0.02 & 0.03 & 23.85 & 22.89 & 9.61 \\ 
%   3C~436 & 0.18 & 16.22 & -0.06 & 0.07 & -0.09 & 0.01 & 4.67 & 19.66 & 2.70 \\ 
%   3C~438 & 0.04 & -7.92 & -0.02 & 0.56 & -0.37 & 0.06 & 5.55 & 19.46 & 1.88 \\ 
%   3C~442 & 0.13 & -47.05 & -0.02 & 0.07 & -0.04 & 0.03 & 1.44 & 43.60 & 1.17 \\ 
%   3C~445 & 0.10 & 57.80 & -0.25 & 0.09 & -0.06 & 0.14 & 0.12 & 12.43 & 10.00 \\ 
%   3C~449 & 0.15 & -17.18 & -0.09 & 0.00 & -0.01 & 0.02 & 0.97 & 17.29 & 1.38 \\ 
%   3C~452 & 0.26 & -75.69 & -0.04 & 0.09 & -0.02 & 0.01 & 2.61 & 18.83 & 2.94 \\ 
%   3C~459 & 0.06 & 24.45 & -0.09 & 0.04 & -0.13 & 0.13 & 2.22 & 18.26 & 10.00 \\ 
%   3C~465 & 0.09 & 28.95 & -0.09 & 0.04 & -0.04 & 0.04 & 2.39 & 17.85 & 1.66 \\ 
  \enddata
  \tablecomments{Properties of the elliptical isophotal fit to each source, including 1-D radial-profile \sersic fit:
    median ellipticity;
    median position angle (East of North);
    minimum value of $a_3/a$;
    maximum value of $a_3/a$;
    minimum value of $a_4/a$;
    maximum value of $a_4/a$.
    scale length (half-light radius) of best-fit model to elliptical isophotes;
    mean surface brightness of model within scale-length, $\langle\mu\rangle_e$;
    \sersic index of model.}
\end{deluxetable}




==> tab5.tex <==
% Table 5: SERSIC RESULTS

\begin{deluxetable}{lrrrrrrrr}
  \tabletypesize{\tiny}
  \tablecolumns{9}
  \tablewidth{0pc}
  \renewcommand{\arraystretch}{.6}
  \tablecaption{\label{tab-sers} 2-D \sersic model fits}
  \tablehead{
  \colhead{Source} &
  \colhead{$M_{H}$(Nuc)} &
  \colhead{$M_{H}$(Host)} &
  \colhead{$R_e$/kpc} &
  \colhead{$\mu_H$} &
  \colhead{$n$} &
  \colhead{$1-\frac{b}{a}$} &
  \colhead{$\theta$} &
  \colhead{$d$}
  }
  \startdata
%    \input{/Users/floyd/3C/Work/idl/sersic}
3C~15 &$...$&$-24.33\pm 0.01$&$8.41\pm 0.05$&$18.86\pm 0.01$&$6.10\pm 0.02$&$0.07\pm 0.00$&$19.33\pm 0.38$&$0.11\pm 0.01$\\
3C~17 &$-21.51$&$-24.19\pm 0.01$&$4.25\pm 0.05$&$17.52\pm 0.00$&$7.49\pm 0.11$&$0.23\pm 0.00$&$20.94\pm 0.31$&$-0.21\pm 0.02$\\
3C~20 &$...$&$-23.61\pm 0.00$&$2.19\pm 0.01$&$16.66\pm 0.00$&$2.70\pm 0.01$&$0.10\pm 0.00$&$-65.53\pm 0.62$&$-0.15\pm 0.01$\\
3C~28 &$-18.71$&$-24.70\pm 0.01$&$11.12\pm 0.07$&$19.10\pm 0.01$&$2.32\pm 0.02$&$0.24\pm 0.00$&$-33.50\pm 0.23$&$-0.26\pm 0.01$\\
3C~29 &$-16.19$&$-23.82\pm 0.01$&$4.24\pm 0.01$&$17.89\pm 0.01$&$1.45\pm 0.00$&$0.04\pm 0.00$&$-81.55\pm 0.00$&$0.08\pm 0.00$\\
3C~31 &$...$&$-23.29\pm 0.00$&$1.72\pm 0.00$&$16.46\pm 0.00$&$1.67\pm 0.00$&$0.12\pm 0.00$&$-32.98\pm 0.08$&$-0.01\pm 0.00$\\
3C~33 &$...$&$-23.43\pm 0.00$&$2.98\pm 0.01$&$17.51\pm 0.00$&$3.60\pm 0.01$&$0.08\pm 0.00$&$-35.60\pm 0.26$&$-0.13\pm 0.01$\\
3C~33.1 &$-20.86$&$-23.84\pm 0.02$&$2.68\pm 0.02$&$16.86\pm 0.02$&$6.41\pm 0.00$&$0.01\pm 0.01$&$54.91\pm 2.56$&$0.00\pm 0.00$\\
3C~35 &$...$&$-24.07\pm 0.00$&$8.38\pm 0.04$&$19.11\pm 0.00$&$4.79\pm 0.01$&$0.28\pm 0.00$&$-66.34\pm 0.07$&$-0.02\pm 0.00$\\
3C~52 &$...$&$-25.06\pm 0.00$&$5.22\pm 0.02$&$17.10\pm 0.00$&$2.49\pm 0.01$&$0.35\pm 0.00$&$10.16\pm 0.18$&$-0.17\pm 0.02$\\
3C~61.1 &$-16.96$&$-22.18\pm 0.11$&$1.73\pm 1.56$&$17.59\pm 0.00$&$2.83\pm 0.00$&$0.13\pm 0.01$&$-2.02\pm 1.22$&$0.41\pm 0.00$\\
3C~66B &$...$&$-23.35\pm 0.01$&$2.93\pm 0.01$&$17.56\pm 0.01$&$2.39\pm 0.01$&$0.07\pm 0.00$&$-59.24\pm 0.34$&$0.00\pm 0.00$\\
3C~71 &$...$&$0.86\pm 0.01$&$1.17\pm 0.01$&$39.77\pm 0.00$&$3.12\pm 0.02$&$0.38\pm 0.00$&$44.99\pm 0.09$&$0.00\pm 0.00$\\
3C~75N &$...$&$-23.35\pm 0.00$&$1.68\pm 0.00$&$16.34\pm 0.00$&$3.68\pm 0.01$&$0.14\pm 0.00$&$-78.88\pm 0.15$&$0.22\pm 0.01$\\
3C~76.1 &$...$&$-22.28\pm 0.00$&$1.31\pm 0.00$&$16.88\pm 0.00$&$2.95\pm 0.00$&$0.16\pm 0.00$&$-48.12\pm 0.12$&$-0.08\pm 0.00$\\
3C~79 &$...$&$-24.42\pm 0.01$&$3.85\pm 0.03$&$17.07\pm 0.01$&$4.27\pm 0.03$&$0.34\pm 0.00$&$13.47\pm 0.28$&$0.07\pm 0.03$\\
3C~83.1 &$...$&$-23.98\pm 0.01$&$2.74\pm 0.01$&$16.78\pm 0.01$&$2.03\pm 0.01$&$0.26\pm 0.00$&$-9.97\pm 0.12$&$0.03\pm 0.01$\\
3C~84 &$-19.25$&$-22.20\pm 0.01$&$1.88\pm 0.01$&$17.74\pm 0.01$&$1.26\pm 0.01$&$0.20\pm 0.00$&$-68.41\pm 0.14$&$0.28\pm 0.01$\\
3C~88 &$...$&$-23.66\pm 0.01$&$10.16\pm 0.05$&$19.94\pm 0.01$&$4.11\pm 0.01$&$0.32\pm 0.00$&$-28.28\pm 0.06$&$0.19\pm 0.01$\\
3C~98 &$...$&$-22.93\pm 0.00$&$2.24\pm 0.00$&$17.39\pm 0.00$&$3.88\pm 0.01$&$0.17\pm 0.00$&$53.26\pm 0.08$&$0.00\pm 0.00$\\
3C~105 &$...$&$-22.88\pm 0.00$&$2.17\pm 0.01$&$17.38\pm 0.00$&$3.22\pm 0.01$&$0.35\pm 0.00$&$51.33\pm 0.11$&$-0.03\pm 0.01$\\
3C~111 &$-23.40$&$-23.03\pm 0.00$&$2.62\pm 0.02$&$17.63\pm 0.00$&$2.10\pm 0.00$&$0.29\pm 0.00$&$18.98\pm 0.53$&$0.00\pm 0.00$\\
3C~123 &$...$&$-25.26\pm 0.05$&$15.44\pm 0.55$&$19.25\pm 0.03$&$4.55\pm 0.00$&$0.08\pm 0.00$&$-80.73\pm 0.80$&$0.06\pm 0.00$\\
3C~129 &$...$&$-23.23\pm 0.00$&$2.36\pm 0.00$&$17.21\pm 0.00$&$1.82\pm 0.00$&$0.15\pm 0.00$&$-45.58\pm 0.07$&$0.07\pm 0.00$\\
3C~129.1 &$...$&$-23.59\pm 0.00$&$3.08\pm 0.01$&$17.42\pm 0.00$&$1.68\pm 0.00$&$0.06\pm 0.00$&$87.02\pm 0.21$&$-0.02\pm 0.00$\\
3C~130 &$...$&$-26.65\pm 0.00$&$7.91\pm 0.01$&$16.41\pm 0.00$&$2.89\pm 0.00$&$0.12\pm 0.00$&$-58.48\pm 0.27$&$-0.02\pm 0.00$\\
3C~132 &$...$&$-24.93\pm 0.00$&$6.48\pm 0.04$&$17.70\pm 0.00$&$3.52\pm 0.02$&$0.21\pm 0.00$&$16.13\pm 0.33$&$0.00\pm 0.00$\\
3C~133 &$-23.11$&$-24.63\pm 0.02$&$4.43\pm 0.04$&$17.17\pm 0.02$&$8.65\pm 0.00$&$0.12\pm 0.00$&$-10.48\pm 0.00$&$0.00\pm 0.00$\\
3C~135 &$...$&$-23.38\pm 0.00$&$3.06\pm 0.01$&$17.61\pm 0.00$&$4.32\pm 0.02$&$0.25\pm 0.00$&$-48.04\pm 0.17$&$0.12\pm 0.01$\\
3C~153 &$...$&$-24.68\pm 0.01$&$5.90\pm 0.07$&$17.75\pm 0.00$&$4.37\pm 0.04$&$0.12\pm 0.00$&$-68.55\pm 1.04$&$0.00\pm 0.00$\\
3C~165 &$-18.70$&$-24.24\pm 0.00$&$3.63\pm 0.03$&$17.13\pm 0.00$&$2.54\pm 0.00$&$0.15\pm 0.00$&$-0.01\pm 0.67$&$0.19\pm 0.00$\\
3C~166 &$-21.02$&$-24.66\pm 0.03$&$24.89\pm 0.06$&$20.89\pm 0.03$&$8.83\pm 0.00$&$0.10\pm 0.01$&$-83.89\pm 1.05$&$0.00\pm 0.00$\\
3C~171 &$-18.47$&$-23.62\pm 0.02$&$2.87\pm 0.04$&$17.23\pm 0.02$&$2.59\pm 0.00$&$0.09\pm 0.00$&$-60.45\pm 1.64$&$0.00\pm 0.00$\\
3C~173.1 &$...$&$-24.57\pm 0.00$&$2.64\pm 0.01$&$16.10\pm 0.00$&$1.80\pm 0.02$&$0.26\pm 0.00$&$14.57\pm 0.62$&$0.23\pm 0.05$\\
3C~180 &$...$&$-24.63\pm 0.00$&$9.77\pm 0.04$&$18.89\pm 0.00$&$2.89\pm 0.01$&$0.45\pm 0.00$&$31.33\pm 0.10$&$0.68\pm 0.02$\\
3C~184.1 &$-20.66$&$-23.16\pm 0.01$&$2.02\pm 0.01$&$16.93\pm 0.01$&$5.89\pm 0.00$&$0.27\pm 0.00$&$44.52\pm 0.65$&$-0.17\pm 0.00$\\
3C~192 &$...$&$-23.17\pm 0.00$&$2.00\pm 0.00$&$16.90\pm 0.00$&$3.41\pm 0.00$&$0.00\pm 0.00$&$-74.83\pm 1.16$&$0.08\pm 0.00$\\
3C~196.1 &$...$&$-25.79\pm 0.71$&$41.00\pm 34.40$&$20.84\pm 0.00$&$3.73\pm 0.00$&$0.32\pm 0.27$&$53.34\pm 32.16$&$0.00\pm 0.00$\\
3C~197.1 &$-18.78$&$-23.62\pm 0.03$&$4.19\pm 0.03$&$18.05\pm 0.03$&$5.03\pm 0.00$&$0.00\pm 0.01$&$-4.98\pm 0.41$&$-0.18\pm 0.00$\\
3C~198 &$-18.53$&$-22.55\pm 0.02$&$3.14\pm 0.01$&$18.50\pm 0.02$&$6.44\pm 0.00$&$0.13\pm 0.00$&$70.70\pm 0.27$&$0.00\pm 0.00$\\
3C~213.1 &$...$&$-23.64\pm 0.00$&$3.84\pm 0.03$&$17.84\pm 0.00$&$3.83\pm 0.03$&$0.41\pm 0.00$&$-60.63\pm 0.21$&$-0.10\pm 0.02$\\
3C~219 &$-20.96$&$-24.67\pm 0.02$&$10.44\pm 0.64$&$18.99\pm 0.00$&$5.09\pm 0.00$&$0.27\pm 0.01$&$-57.17\pm 0.22$&$-0.10\pm 0.00$\\
3C~223 &$...$&$-23.88\pm 0.01$&$6.88\pm 0.12$&$18.87\pm 0.00$&$5.18\pm 0.07$&$0.19\pm 0.00$&$65.25\pm 0.41$&$-0.57\pm 0.01$\\
3C~223.1 &$-16.66$&$-24.66\pm 0.01$&$15.79\pm 0.01$&$19.90\pm 0.01$&$9.73\pm 0.00$&$0.42\pm 0.00$&$40.18\pm 0.05$&$-0.41\pm 0.00$\\
3C~227 &$-22.43$&$-22.66\pm 0.01$&$2.48\pm 0.01$&$17.89\pm 0.01$&$2.68\pm 0.03$&$0.15\pm 0.00$&$-3.34\pm 0.26$&$-0.22\pm 0.01$\\
3C~234 &$-23.71$&$-23.36\pm 0.00$&$2.95\pm 0.01$&$17.56\pm 0.00$&$1.59\pm 0.00$&$0.08\pm 0.00$&$-74.91\pm 1.51$&$-0.12\pm 0.00$\\
3C~236 &$...$&$-24.04\pm 0.00$&$4.64\pm 0.01$&$17.86\pm 0.00$&$3.90\pm 0.01$&$0.42\pm 0.00$&$47.52\pm 0.06$&$0.17\pm 0.01$\\
3C~258 &$...$&$-20.11\pm 0.02$&$1.19\pm 0.03$&$18.84\pm 0.00$&$3.26\pm 0.12$&$0.27\pm 0.01$&$-35.04\pm 1.98$&$0.00\pm 0.00$\\
3C~264 &$...$&$-22.38\pm 0.02$&$1.12\pm 0.00$&$16.45\pm 0.02$&$1.63\pm 0.00$&$0.02\pm 0.00$&$-8.29\pm 0.65$&$0.06\pm 0.00$\\
3C~270 &$...$&$-22.63\pm 0.05$&$1.49\pm 0.10$&$16.81\pm 0.00$&$1.96\pm 0.00$&$0.27\pm 0.00$&$-22.24\pm 0.97$&$0.00\pm 0.00$\\
3C~272.1 &$...$&$-21.02\pm 0.00$&$0.42\pm 0.00$&$15.69\pm 0.00$&$1.44\pm 0.00$&$0.19\pm 0.00$&$-52.87\pm 0.03$&$0.08\pm 0.00$\\
3C~274 &$-15.87$&$-22.55\pm 0.08$&$1.39\pm 0.04$&$16.74\pm 0.08$&$1.24\pm 0.01$&$0.02\pm 0.00$&$-15.61\pm 0.33$&$0.15\pm 0.00$\\
3C~277.3 &$...$&$-23.42\pm 0.00$&$3.19\pm 0.01$&$17.67\pm 0.00$&$2.51\pm 0.01$&$0.07\pm 0.00$&$-21.38\pm 0.35$&$-0.06\pm 0.01$\\
3C~284 &$...$&$-24.54\pm 0.00$&$4.48\pm 0.02$&$17.28\pm 0.00$&$3.40\pm 0.02$&$0.07\pm 0.00$&$30.56\pm 1.10$&$0.00\pm 0.00$\\
3C~285 &$...$&$-23.61\pm 0.01$&$7.30\pm 0.06$&$19.28\pm 0.01$&$3.13\pm 0.02$&$0.36\pm 0.00$&$-57.18\pm 0.14$&$-0.19\pm 0.01$\\
3C~287.1 &$-23.16$&$-24.14\pm 0.01$&$5.28\pm 0.06$&$18.04\pm 0.00$&$5.94\pm 0.08$&$0.15\pm 0.00$&$34.92\pm 0.79$&$0.00\pm 0.00$\\
3C~288 &$...$&$-25.16\pm 0.00$&$8.13\pm 0.02$&$17.96\pm 0.00$&$1.43\pm 0.01$&$0.05\pm 0.00$&$-39.33\pm 1.00$&$-0.15\pm 0.01$\\
3C~293 &$...$&$-24.40\pm 0.01$&$18.45\pm 0.12$&$20.50\pm 0.01$&$4.15\pm 0.01$&$0.46\pm 0.00$&$58.41\pm 0.05$&$0.00\pm 0.01$\\
3C~296 &$...$&$-25.22\pm 0.00$&$14.93\pm 0.02$&$19.22\pm 0.00$&$4.41\pm 0.00$&$0.31\pm 0.00$&$-32.87\pm 0.08$&$0.00\pm 0.00$\\
3C~300 &$...$&$-23.52\pm 0.01$&$2.84\pm 0.03$&$17.32\pm 0.00$&$3.10\pm 0.05$&$0.31\pm 0.01$&$-51.10\pm 0.99$&$0.00\pm 0.00$\\
3C~303 &$-21.83$&$-23.93\pm 0.00$&$3.61\pm 0.01$&$17.42\pm 0.00$&$4.00\pm 0.00$&$0.12\pm 0.00$&$-16.27\pm 0.47$&$0.00\pm 0.00$\\
3C~305 &$-18.97$&$-24.42\pm 0.02$&$14.02\pm 0.09$&$19.88\pm 0.02$&$5.96\pm 0.00$&$0.26\pm 0.00$&$68.91\pm 0.15$&$-0.11\pm 0.00$\\
3C~310 &$...$&$-22.93\pm 0.00$&$3.60\pm 0.01$&$18.42\pm 0.00$&$2.74\pm 0.01$&$0.25\pm 0.00$&$86.85\pm 0.10$&$-0.07\pm 0.01$\\
3C~314.1 &$...$&$-22.96\pm 0.00$&$3.67\pm 0.01$&$18.43\pm 0.00$&$3.31\pm 0.01$&$0.40\pm 0.00$&$70.99\pm 0.14$&$0.06\pm 0.02$\\
3C~315 &$...$&$-23.20\pm 0.00$&$2.66\pm 0.01$&$17.49\pm 0.00$&$4.52\pm 0.02$&$0.47\pm 0.00$&$35.38\pm 0.11$&$-0.15\pm 0.01$\\
3C~317 &$-18.01$&$-24.13\pm 0.04$&$21.19\pm 0.05$&$21.06\pm 0.04$&$4.00\pm 0.00$&$0.25\pm 0.01$&$63.91\pm 0.32$&$-0.30\pm 0.00$\\
3C~319 &$...$&$-23.62\pm 0.04$&$6.76\pm 1.62$&$19.10\pm 0.00$&$7.34\pm 0.00$&$0.22\pm 0.00$&$-42.45\pm 0.54$&$-0.18\pm 0.00$\\
3C~321 &$...$&$-23.97\pm 0.00$&$3.31\pm 0.01$&$17.20\pm 0.00$&$2.53\pm 0.01$&$0.07\pm 0.00$&$-76.34\pm 0.82$&$0.02\pm 0.01$\\
3C~323.1 &$-25.34$&$-24.05\pm 0.00$&$3.13\pm 0.02$&$17.00\pm 0.00$&$1.70\pm 0.00$&$0.19\pm 0.00$&$62.61\pm 0.73$&$0.08\pm 0.00$\\
3C~326 &$...$&$-22.99\pm 0.00$&$2.17\pm 0.00$&$17.26\pm 0.00$&$3.47\pm 0.01$&$0.45\pm 0.00$&$-72.75\pm 0.08$&$0.00\pm 0.00$\\
3C~332 &$-23.61$&$-23.37\pm 0.02$&$3.20\pm 0.02$&$17.73\pm 0.02$&$1.72\pm 0.00$&$0.01\pm 0.00$&$-53.83\pm 4.21$&$-0.09\pm 0.00$\\
3C~338 &$...$&$-28.05\pm 0.47$&$194.30\pm 44.85$&$21.96\pm 0.41$&$3.72\pm 0.20$&$0.22\pm 0.00$&$47.45\pm 0.18$&$0.48\pm 0.02$\\
3C~346 &$-19.00$&$-23.78\pm 0.01$&$5.02\pm 0.07$&$18.29\pm 0.00$&$7.35\pm 0.08$&$0.18\pm 0.00$&$-48.43\pm 0.65$&$0.00\pm 0.00$\\
3C~348 &$...$&$-24.25\pm 0.00$&$10.13\pm 0.03$&$19.35\pm 0.00$&$1.06\pm 0.00$&$0.32\pm 0.00$&$-59.47\pm 0.16$&$-0.05\pm 0.01$\\
3C~349 &$-20.41$&$-23.49\pm 0.01$&$3.37\pm 0.02$&$17.72\pm 0.01$&$3.54\pm 0.04$&$0.44\pm 0.00$&$21.21\pm 0.20$&$0.12\pm 0.03$\\
3C~353 &$...$&$-22.99\pm 0.00$&$2.48\pm 0.00$&$17.55\pm 0.00$&$4.00\pm 0.00$&$0.03\pm 0.00$&$77.45\pm 0.62$&$0.00\pm 0.00$\\
3C~357 &$...$&$-24.98\pm 0.01$&$11.34\pm 0.10$&$18.86\pm 0.00$&$5.34\pm 0.03$&$0.29\pm 0.00$&$83.67\pm 0.14$&$0.00\pm 0.00$\\
3C~371 &$-23.07$&$-23.37\pm 0.01$&$2.31\pm 0.01$&$17.02\pm 0.01$&$3.81\pm 0.05$&$0.07\pm 0.00$&$71.56\pm 0.24$&$0.07\pm 0.00$\\
3C~379.1 &$-19.24$&$-24.96\pm 0.00$&$6.31\pm 0.03$&$17.61\pm 0.00$&$2.98\pm 0.02$&$0.10\pm 0.00$&$-45.01\pm 0.64$&$0.00\pm 0.00$\\
3C~381 &$-19.10$&$-23.77\pm 0.00$&$2.84\pm 0.01$&$17.07\pm 0.00$&$3.62\pm 0.02$&$0.18\pm 0.00$&$64.63\pm 0.30$&$-0.05\pm 0.01$\\
3C~382 &$-23.40$&$-24.29\pm 0.01$&$4.66\pm 0.04$&$17.61\pm 0.01$&$5.81\pm 0.06$&$0.31\pm 0.00$&$88.99\pm 0.05$&$0.00\pm 0.00$\\
3C~386 &$-19.48$&$-22.73\pm 0.00$&$1.76\pm 0.00$&$17.07\pm 0.00$&$2.50\pm 0.01$&$0.13\pm 0.00$&$-75.63\pm 0.13$&$-0.05\pm 0.00$\\
3C~388 &$...$&$-24.66\pm 0.00$&$7.76\pm 0.02$&$18.36\pm 0.00$&$1.83\pm 0.01$&$0.16\pm 0.00$&$43.88\pm 0.16$&$-0.15\pm 0.01$\\
3C~390.3 &$-22.79$&$-23.04\pm 0.01$&$2.07\pm 0.00$&$17.10\pm 0.01$&$3.13\pm 0.04$&$0.17\pm 0.00$&$79.90\pm 0.15$&$-0.13\pm 0.01$\\
3C~401 &$...$&$-24.77\pm 0.02$&$18.88\pm 0.31$&$20.18\pm 0.01$&$3.70\pm 0.04$&$0.18\pm 0.00$&$-85.91\pm 0.40$&$0.34\pm 0.03$\\
3C~402 &$...$&$-22.94\pm 0.00$&$1.84\pm 0.00$&$16.96\pm 0.00$&$2.86\pm 0.00$&$0.18\pm 0.00$&$34.29\pm 0.06$&$0.02\pm 0.00$\\
3C~403 &$...$&$-24.44\pm 0.05$&$7.98\pm 0.05$&$18.64\pm 0.05$&$4.56\pm 0.00$&$0.26\pm 0.01$&$36.68\pm 2.32$&$0.05\pm 0.00$\\
3C~403.1 &$...$&$-22.73\pm 0.00$&$1.33\pm 0.00$&$16.46\pm 0.00$&$3.48\pm 0.01$&$0.19\pm 0.00$&$-27.94\pm 0.16$&$-0.07\pm 0.01$\\
3C~405 &$-16.23$&$-22.98\pm 0.17$&$3.84\pm 0.13$&$18.50\pm 0.17$&$0.76\pm 0.00$&$0.21\pm 0.01$&$-16.97\pm 2.17$&$0.00\pm 0.00$\\
3C~410 &$-24.63$&$-25.08\pm 0.02$&$5.62\pm 0.13$&$17.23\pm 0.00$&$5.87\pm 0.20$&$0.16\pm 0.01$&$85.91\pm 0.82$&$-0.39\pm 0.03$\\
3C~424 &$-17.13$&$-23.32\pm 0.01$&$7.58\pm 0.13$&$19.65\pm 0.00$&$6.81\pm 0.08$&$0.08\pm 0.00$&$84.81\pm 0.85$&$0.00\pm 0.00$\\
3C~430 &$...$&$-23.86\pm 0.00$&$3.67\pm 0.01$&$17.53\pm 0.00$&$4.06\pm 0.01$&$0.37\pm 0.00$&$-73.44\pm 0.06$&$-0.03\pm 0.00$\\
3C~433 &$-21.16$&$-24.28\pm 0.01$&$6.61\pm 0.08$&$18.40\pm 0.00$&$2.36\pm 0.04$&$0.41\pm 0.00$&$-29.51\pm 0.24$&$-0.26\pm 0.02$\\
3C~436 &$...$&$-24.46\pm 0.00$&$4.87\pm 0.02$&$17.55\pm 0.00$&$2.91\pm 0.01$&$0.23\pm 0.00$&$11.80\pm 0.27$&$0.13\pm 0.02$\\
3C~438 &$...$&$-25.07\pm 0.01$&$6.37\pm 0.03$&$17.53\pm 0.01$&$2.57\pm 0.02$&$0.07\pm 0.00$&$-16.52\pm 0.94$&$-0.24\pm 0.02$\\
3C~442 &$...$&$-22.26\pm 0.00$&$1.55\pm 0.00$&$17.26\pm 0.00$&$1.28\pm 0.00$&$0.12\pm 0.00$&$-47.59\pm 0.17$&$-0.07\pm 0.00$\\
3C~445 &$-22.62$&$-22.21\pm 0.01$&$1.75\pm 0.00$&$17.57\pm 0.01$&$3.74\pm 0.36$&$0.15\pm 0.00$&$77.94\pm 0.00$&$0.10\pm 0.00$\\
3C~449 &$...$&$-22.36\pm 0.00$&$1.16\pm 0.00$&$16.54\pm 0.00$&$1.55\pm 0.00$&$0.18\pm 0.00$&$-3.86\pm 0.08$&$0.02\pm 0.00$\\
3C~452 &$...$&$-23.75\pm 0.00$&$3.78\pm 0.01$&$17.70\pm 0.00$&$3.84\pm 0.01$&$0.28\pm 0.00$&$-74.87\pm 0.09$&$0.00\pm 0.00$\\
3C~459 &$-21.86$&$-24.61\pm 0.01$&$3.17\pm 0.04$&$16.47\pm 0.00$&$9.79\pm 0.14$&$0.05\pm 0.00$&$-61.31\pm 0.96$&$-0.24\pm 0.02$\\
3C~465 &$...$&$-24.09\pm 0.01$&$4.04\pm 0.02$&$17.51\pm 0.01$&$2.56\pm 0.01$&$0.19\pm 0.00$&$30.09\pm 0.11$&$0.00\pm 0.00$\\

%   3C~15&   $...$    &$-24.33\pm 0.01$&$8.41\pm 0.05$&$20.78\pm 0.01$&$6.10\pm 0.02$&$0.07\pm 0.00$&$19.33\pm 0.38$&$0.11\pm 0.01$\\
%   3C~17&   $-21.51$ &$-24.19\pm 0.01$&$4.25\pm 0.05$&$20.11\pm 0.00$&$7.49\pm 0.11$&$0.23\pm 0.00$&$20.94\pm 0.31$&$-0.21\pm 0.02$\\
%   3C~20&   $...$    &$-23.61\pm 0.00$&$2.19\pm 0.01$&$18.55\pm 0.00$&$2.70\pm 0.01$&$0.10\pm 0.00$&$-65.53\pm 0.62$&$-0.15\pm 0.01$\\
%   3C~28&   $-18.71$ &$-24.70\pm 0.01$&$11.12\pm 0.07$&$20.99\pm 0.01$&$2.32\pm 0.02$&$0.24\pm 0.00$&$-33.50\pm 0.23$&$-0.26\pm 0.01$\\
%   3C~29&   $-16.19$ &$-23.82\pm 0.01$&$4.24\pm 0.01$&$18.95\pm 0.01$&$1.45\pm 0.00$&$0.04\pm 0.00$&$-81.55\pm 0.00$&$0.08\pm 0.00$\\
%   3C~31&   $...$    &$-23.29\pm 0.00$&$1.72\pm 0.00$&$17.48\pm 0.00$&$1.67\pm 0.00$&$0.12\pm 0.00$&$-32.98\pm 0.08$&$-0.01\pm 0.00$\\
%   3C~33&   $...$    &$-23.43\pm 0.00$&$2.98\pm 0.01$&$19.10\pm 0.00$&$3.60\pm 0.01$&$0.08\pm 0.00$&$-35.60\pm 0.26$&$-0.13\pm 0.01$\\
%   3C~33.1& $-20.86$ &$-23.84\pm 0.02$&$2.68\pm 0.02$&$19.23\pm 0.02$&$6.41\pm 0.00$&$0.01\pm 0.01$&$54.91\pm 2.56$&$0.00\pm 0.00$\\
%   3C~35&   $...$    &$-24.07\pm 0.00$&$8.38\pm 0.04$&$20.88\pm 0.00$&$4.79\pm 0.01$&$0.28\pm 0.00$&$-66.34\pm 0.07$&$-0.02\pm 0.00$\\
%   3C~52&   $...$    &$-25.06\pm 0.00$&$5.22\pm 0.02$&$19.33\pm 0.00$&$2.49\pm 0.01$&$0.35\pm 0.00$&$10.16\pm 0.18$&$-0.17\pm 0.02$\\
%   3C~61.1& $-16.96$ &$-22.18\pm 0.11$&$1.73\pm 1.56$&$19.54\pm 0.00$&$2.83\pm 0.00$&$0.13\pm 0.01$&$-2.02\pm 1.22$&$0.41\pm 0.00$\\
%   3C~66B&  $...$    &$-23.35\pm 0.01$&$2.93\pm 0.01$&$18.77\pm 0.01$&$2.39\pm 0.01$&$0.07\pm 0.00$&$-59.24\pm 0.34$&$0.00\pm 0.00$\\
%   3C~71$^{(a)}$ & $...$  &$...$      &$...$         &$...$          &$3.08\pm 0.02$&$0.39\pm 0.00$&$44.44\pm 0.10$&$-0.37\pm 0.00$\\ 
%   3C~75N&  $64.57$  &$-23.35\pm 0.00$&$1.68\pm 0.00$&$17.80\pm 0.00$&$3.68\pm 0.01$&$0.14\pm 0.00$&$-78.88\pm 0.15$&$0.00\pm 0.01$\\
%   3C~76.1& $...$    &$-22.28\pm 0.00$&$1.31\pm 0.00$&$18.25\pm 0.00$&$2.95\pm 0.00$&$0.16\pm 0.00$&$-48.12\pm 0.12$&$0.22\pm 0.00$\\
%   3C~79&   $...$    &$-24.42\pm 0.01$&$3.85\pm 0.03$&$19.49\pm 0.01$&$4.27\pm 0.03$&$0.34\pm 0.00$&$13.47\pm 0.28$&$-0.08\pm 0.03$\\
%   3C~83.1& $...$    &$-23.98\pm 0.01$&$2.74\pm 0.01$&$17.93\pm 0.01$&$2.03\pm 0.01$&$0.26\pm 0.00$&$-9.97\pm 0.12$&$0.07\pm 0.01$\\
%   3C~84&   $...$    &$-22.20\pm 0.01$&$1.88\pm 0.01$&$18.62\pm 0.01$&$1.26\pm 0.01$&$0.20\pm 0.00$&$-68.41\pm 0.14$&$0.03\pm 0.01$\\
%   3C~88&   $64.10$  &$-23.66\pm 0.01$&$10.16\pm 0.05$&$21.48\pm 0.01$&$4.11\pm 0.01$&$0.32\pm 0.00$&$-28.28\pm 0.06$&$0.28\pm 0.01$\\
%   3C~98&   $...$    &$-22.93\pm 0.00$&$2.24\pm 0.00$&$18.89\pm 0.00$&$3.88\pm 0.01$&$0.17\pm 0.00$&$53.26\pm 0.08$&$0.19\pm 0.00$\\
%   3C~105&  $...$    &$-22.88\pm 0.00$&$2.17\pm 0.01$&$19.03\pm 0.00$&$3.22\pm 0.01$&$0.35\pm 0.00$&$51.33\pm 0.11$&$0.00\pm 0.01$\\
%   3C~111&  $...$    &$-23.03\pm 0.00$&$2.62\pm 0.02$&$18.89\pm 0.00$&$2.10\pm 0.00$&$0.29\pm 0.00$&$18.98\pm 0.53$&$-0.03\pm 0.00$\\
%   3C~123&  $58.86$  &$-25.26\pm 0.05$&$15.44\pm 0.55$&$21.57\pm 0.03$&$4.55\pm 0.00$&$0.08\pm 0.00$&$-80.73\pm 0.80$&$0.00\pm 0.00$\\
%   3C~129&  $...$    &$-23.23\pm 0.00$&$2.36\pm 0.00$&$18.29\pm 0.00$&$1.82\pm 0.00$&$0.15\pm 0.00$&$-45.58\pm 0.07$&$0.06\pm 0.00$\\
%   3C~129.1&$...$    &$-23.59\pm 0.00$&$3.08\pm 0.01$&$18.46\pm 0.00$&$1.68\pm 0.00$&$0.06\pm 0.00$&$87.02\pm 0.21$&$0.07\pm 0.00$\\
%   3C~130&  $...$    &$-26.65\pm 0.00$&$7.91\pm 0.01$&$18.08\pm 0.00$&$2.89\pm 0.00$&$0.12\pm 0.00$&$-58.48\pm 0.27$&$-0.02\pm 0.00$\\
%   3C~132&  $...$    &$-24.93\pm 0.00$&$6.48\pm 0.04$&$19.87\pm 0.00$&$3.52\pm 0.02$&$0.21\pm 0.00$&$16.13\pm 0.33$&$-0.02\pm 0.00$\\
%   3C~133&  $...$    &$-24.63\pm 0.02$&$4.43\pm 0.04$&$20.04\pm 0.02$&$8.65\pm 0.00$&$0.12\pm 0.00$&$-10.48\pm 0.00$&$0.00\pm 0.00$\\
%   3C~135&  $60.73$  &$-23.38\pm 0.00$&$3.06\pm 0.01$&$19.57\pm 0.00$&$4.32\pm 0.02$&$0.25\pm 0.00$&$-48.04\pm 0.17$&$0.00\pm 0.01$\\
%   3C~153&  $...$    &$-24.68\pm 0.01$&$5.90\pm 0.07$&$20.24\pm 0.00$&$4.37\pm 0.04$&$0.12\pm 0.00$&$-68.55\pm 1.04$&$0.12\pm 0.00$\\
%   3C~165&  $...$    &$-24.24\pm 0.00$&$3.63\pm 0.03$&$19.41\pm 0.00$&$2.54\pm 0.00$&$0.15\pm 0.00$&$-0.01\pm 0.67$&$0.00\pm 0.00$\\
%   3C~166&  $-21.02$ &$-24.66\pm 0.03$&$24.89\pm 0.06$&$23.65\pm 0.03$&$8.83\pm 0.00$&$0.10\pm 0.01$&$-83.89\pm 1.05$&$0.19\pm 0.00$\\
%   3C~171&  $-18.47$ &$-23.62\pm 0.02$&$2.87\pm 0.04$&$19.33\pm 0.02$&$2.59\pm 0.00$&$0.09\pm 0.00$&$-60.45\pm 1.64$&$0.00\pm 0.00$\\
%   3C~173.1&$58.61$  &$-24.57\pm 0.00$&$2.64\pm 0.01$&$18.20\pm 0.00$&$1.80\pm 0.02$&$0.26\pm 0.00$&$14.57\pm 0.62$&$0.00\pm 0.05$\\
%   3C~180&  $...$    &$-24.63\pm 0.00$&$9.77\pm 0.04$&$20.98\pm 0.00$&$2.89\pm 0.01$&$0.45\pm 0.00$&$31.33\pm 0.10$&$0.23\pm 0.02$\\
%   3C~184.1&$...$    &$-23.16\pm 0.01$&$2.02\pm 0.01$&$19.01\pm 0.01$&$5.89\pm 0.00$&$0.27\pm 0.00$&$44.52\pm 0.65$&$0.68\pm 0.00$\\
%   3C~192&  $62.60$  &$-23.17\pm 0.00$&$2.00\pm 0.00$&$18.46\pm 0.00$&$3.41\pm 0.00$&$0.00\pm 0.00$&$-74.83\pm 1.16$&$-0.17\pm 0.00$\\
%   3C~196.1&$...$    &$-25.79\pm 0.71$&$41.00\pm 34.40$&$22.98\pm 0.00$&$3.73\pm 0.00$&$0.32\pm 0.27$&$53.34\pm 32.16$&$0.08\pm 0.00$\\
%   3C~197.1&$...$    &$-23.62\pm 0.03$&$4.19\pm 0.03$&$20.10\pm 0.03$&$5.03\pm 0.00$&$0.00\pm 0.01$&$-4.98\pm 0.41$&$0.00\pm 0.00$\\
%   3C~198&  $-18.53$ &$-22.55\pm 0.02$&$3.14\pm 0.01$&$20.48\pm 0.02$&$6.44\pm 0.00$&$0.13\pm 0.00$&$70.70\pm 0.27$&$-0.18\pm 0.00$\\
%   3C~213.1&$59.71$  &$-23.64\pm 0.00$&$3.84\pm 0.03$&$19.99\pm 0.00$&$3.83\pm 0.03$&$0.41\pm 0.00$&$-60.63\pm 0.21$&$0.00\pm 0.02$\\
%   3C~219&  $...$    &$-24.67\pm 0.02$&$10.44\pm 0.64$&$21.21\pm 0.00$&$5.09\pm 0.00$&$0.27\pm 0.01$&$-57.17\pm 0.22$&$-0.10\pm 0.00$\\
%   3C~223&  $60.62$  &$-23.88\pm 0.01$&$6.88\pm 0.12$&$20.95\pm 0.00$&$5.18\pm 0.07$&$0.19\pm 0.00$&$65.25\pm 0.41$&$-0.10\pm 0.01$\\
%   3C~223.1&$...$    &$-24.66\pm 0.01$&$15.79\pm 0.01$&$22.21\pm 0.01$&$9.73\pm 0.00$&$0.42\pm 0.00$&$40.18\pm 0.05$&$-0.57\pm 0.00$\\
%   3C~227&  $-22.43$ &$-22.66\pm 0.01$&$2.48\pm 0.01$&$19.43\pm 0.01$&$2.68\pm 0.03$&$0.15\pm 0.00$&$-3.34\pm 0.26$&$-0.41\pm 0.01$\\
%   3C~234&  $-23.71$ &$-23.36\pm 0.00$&$2.95\pm 0.01$&$19.21\pm 0.00$&$1.59\pm 0.00$&$0.08\pm 0.00$&$-74.91\pm 1.51$&$-0.22\pm 0.00$\\
%   3C~236&  $61.43$  &$-24.04\pm 0.00$&$4.64\pm 0.01$&$19.65\pm 0.00$&$3.90\pm 0.01$&$0.42\pm 0.00$&$47.52\pm 0.06$&$-0.12\pm 0.01$\\
%   3C~258$^{(b)}$ &  $...$    &$-20.11\pm 0.02$&$1.19\pm 0.03$&$18.84\pm0.03$&$3.26\pm0.12$&$0.27\pm0.01$&$-35.04\pm1.98$&$0.00\pm 0.00$\\ 
%   3C~264&  $...$    &$-22.38\pm 0.02$&$1.12\pm 0.00$&$17.47\pm 0.02$&$1.63\pm 0.00$&$0.02\pm 0.00$&$-8.29\pm 0.65$&$0.17\pm 0.00$\\
%   3C~270&  $...$    &$-22.63\pm 0.05$&$1.49\pm 0.10$&$17.87\pm 0.00$&$1.96\pm 0.00$&$0.27\pm 0.00$&$-22.24\pm 0.97$&$0.00\pm 0.00$\\
%   3C~272.1&$...$    &$-21.02\pm 0.00$&$0.42\pm 0.00$&$16.58\pm 0.00$&$1.44\pm 0.00$&$0.19\pm 0.00$&$-52.87\pm 0.03$&$0.06\pm 0.00$\\
%   3C~274&  $...$    &$-22.55\pm 0.08$&$1.39\pm 0.04$&$17.56\pm 0.08$&$1.24\pm 0.01$&$0.02\pm 0.00$&$-15.61\pm 0.33$&$0.00\pm 0.00$\\
%   3C~277.3&$...$    &$-23.42\pm 0.00$&$3.19\pm 0.01$&$19.17\pm 0.00$&$2.51\pm 0.01$&$0.07\pm 0.00$&$-21.38\pm 0.35$&$0.08\pm 0.01$\\
%   3C~284&  $59.17$  &$-24.54\pm 0.00$&$4.48\pm 0.02$&$19.52\pm 0.00$&$3.40\pm 0.02$&$0.07\pm 0.00$&$30.56\pm 1.10$&$0.15\pm 0.00$\\
%   3C~285&  $...$    &$-23.61\pm 0.01$&$7.30\pm 0.06$&$20.87\pm 0.01$&$3.13\pm 0.02$&$0.36\pm 0.00$&$-57.18\pm 0.14$&$-0.06\pm 0.01$\\
%   3C~287.1&$...$    &$-24.14\pm 0.01$&$5.28\pm 0.06$&$20.49\pm 0.00$&$5.94\pm 0.08$&$0.15\pm 0.00$&$34.92\pm 0.79$&$0.00\pm 0.00$\\
%   3C~288&  $...$    &$-25.16\pm 0.00$&$8.13\pm 0.02$&$19.79\pm 0.00$&$1.43\pm 0.01$&$0.05\pm 0.00$&$-39.33\pm 1.00$&$-0.19\pm 0.01$\\
%   3C~293&  $63.25$  &$-24.40\pm 0.01$&$18.45\pm 0.12$&$22.10\pm 0.01$&$4.15\pm 0.01$&$0.46\pm 0.00$&$58.41\pm 0.05$&$0.00\pm 0.01$\\
%   3C~296&  $...$    &$-25.22\pm 0.00$&$14.93\pm 0.02$&$20.76\pm 0.00$&$4.41\pm 0.00$&$0.31\pm 0.00$&$-32.87\pm 0.08$&$-0.15\pm 0.00$\\
%   3C~300&  $...$    &$-23.52\pm 0.01$&$2.84\pm 0.03$&$19.62\pm 0.00$&$3.10\pm 0.05$&$0.31\pm 0.01$&$-51.10\pm 0.99$&$0.00\pm 0.00$\\
%   3C~303&  $...$    &$-23.93\pm 0.00$&$3.61\pm 0.01$&$19.39\pm 0.00$&$4.00\pm 0.00$&$0.12\pm 0.00$&$-16.27\pm 0.47$&$0.00\pm 0.00$\\
%   3C~305&  $...$    &$-24.42\pm 0.02$&$14.02\pm 0.09$&$21.66\pm 0.02$&$5.96\pm 0.00$&$0.26\pm 0.00$&$68.91\pm 0.15$&$0.00\pm 0.00$\\
%   3C~310&  $62.81$  &$-22.93\pm 0.00$&$3.60\pm 0.01$&$19.85\pm 0.00$&$2.74\pm 0.01$&$0.25\pm 0.00$&$86.85\pm 0.10$&$0.00\pm 0.01$\\
%   3C~314.1&$60.95$  &$-22.96\pm 0.00$&$3.67\pm 0.01$&$20.22\pm 0.00$&$3.31\pm 0.01$&$0.40\pm 0.00$&$70.99\pm 0.14$&$-0.11\pm 0.02$\\
%   3C~315&  $...$    &$-23.20\pm 0.00$&$2.66\pm 0.01$&$19.39\pm 0.00$&$4.52\pm 0.02$&$0.47\pm 0.00$&$35.38\pm 0.11$&$-0.07\pm 0.01$\\
%   3C~317&  $...$    &$-24.13\pm 0.04$&$21.19\pm 0.05$&$22.61\pm 0.04$&$4.00\pm 0.00$&$0.25\pm 0.01$&$63.91\pm 0.32$&$0.06\pm 0.00$\\
%   3C~319&  $...$    &$-23.62\pm 0.04$&$6.76\pm 1.62$&$21.57\pm 0.00$&$7.34\pm 0.00$&$0.22\pm 0.00$&$-42.45\pm 0.54$&$-0.15\pm 0.00$\\
%   3C~321&  $61.46$  &$-23.97\pm 0.00$&$3.31\pm 0.01$&$18.76\pm 0.00$&$2.53\pm 0.01$&$0.07\pm 0.00$&$-76.34\pm 0.82$&$-0.30\pm 0.01$\\
%   3C~323.1&$...$    &$-24.05\pm 0.00$&$3.13\pm 0.02$&$18.97\pm 0.00$&$1.70\pm 0.00$&$0.19\pm 0.00$&$62.61\pm 0.73$&$-0.18\pm 0.00$\\
%   3C~326&  $...$    &$-22.99\pm 0.00$&$2.17\pm 0.00$&$18.95\pm 0.00$&$3.47\pm 0.01$&$0.45\pm 0.00$&$-72.75\pm 0.08$&$0.02\pm 0.00$\\
%   3C~332&  $-23.61$ &$-23.37\pm 0.02$&$3.20\pm 0.02$&$19.30\pm 0.02$&$1.72\pm 0.00$&$0.01\pm 0.00$&$-53.83\pm 4.21$&$0.08\pm 0.00$\\
%   3C~338&  $...$    &$-28.05\pm 0.47$&$194.30\pm 45$&$21.96\pm 0.52$&$3.72\pm 0.20$&$0.22\pm 0.00$&$47.45\pm 0.18 $&$0.48\pm 0.02$\\ 
%   3C~346&  $...$    &$-23.78\pm 0.01$&$5.02\pm 0.07$&$20.65\pm 0.00$&$7.35\pm 0.08$&$0.18\pm 0.00$&$-48.43\pm 0.65$&$0.00\pm 0.00$\\
%   3C~348&  $60.26$  &$-24.25\pm 0.00$&$10.13\pm 0.03$&$20.70\pm 0.00$&$1.06\pm 0.00$&$0.32\pm 0.00$&$-59.47\pm 0.16$&$-0.09\pm 0.01$\\
%   3C~349&  $...$    &$-23.49\pm 0.01$&$3.37\pm 0.02$&$19.85\pm 0.01$&$3.54\pm 0.04$&$0.44\pm 0.00$&$21.21\pm 0.20$&$0.48\pm 0.03$\\
%   3C~353&  $63.92$  &$-22.99\pm 0.00$&$2.48\pm 0.00$&$19.07\pm 0.00$&$4.00\pm 0.00$&$0.03\pm 0.00$&$77.45\pm 0.62$&$0.00\pm 0.00$\\
%   3C~357&  $...$    &$-24.98\pm 0.01$&$11.34\pm 0.10$&$21.07\pm 0.00$&$5.34\pm 0.03$&$0.29\pm 0.00$&$83.67\pm 0.14$&$-0.05\pm 0.00$\\
%   3C~371&  $-23.07$ &$-23.37\pm 0.01$&$2.31\pm 0.01$&$18.60\pm 0.01$&$3.81\pm 0.05$&$0.07\pm 0.00$&$71.56\pm 0.24$&$0.12\pm 0.00$\\
%   3C~379.1&$...$    &$-24.96\pm 0.00$&$6.31\pm 0.03$&$19.84\pm 0.00$&$2.98\pm 0.02$&$0.10\pm 0.00$&$-45.01\pm 0.64$&$0.00\pm 0.00$\\
%   3C~381&  $...$    &$-23.77\pm 0.00$&$2.84\pm 0.01$&$19.05\pm 0.00$&$3.62\pm 0.02$&$0.18\pm 0.00$&$64.63\pm 0.30$&$0.00\pm 0.01$\\
%   3C~382&  $-23.40$ &$-24.29\pm 0.01$&$4.66\pm 0.04$&$19.44\pm 0.01$&$5.81\pm 0.06$&$0.31\pm 0.00$&$88.99\pm 0.05$&$0.07\pm 0.00$\\
%   3C~386&  $-19.48$ &$-22.73\pm 0.00$&$1.76\pm 0.00$&$18.29\pm 0.00$&$2.50\pm 0.01$&$0.13\pm 0.00$&$-75.63\pm 0.13$&$0.00\pm 0.00$\\
%   3C~388&  $61.59$  &$-24.66\pm 0.00$&$7.76\pm 0.02$&$19.73\pm 0.00$&$1.83\pm 0.01$&$0.16\pm 0.00$&$43.88\pm 0.16$&$-0.05\pm 0.01$\\
%   3C~390.3&$-22.79$ &$-23.04\pm 0.01$&$2.07\pm 0.00$&$18.61\pm 0.01$&$3.13\pm 0.04$&$0.17\pm 0.00$&$79.90\pm 0.15$&$0.00\pm 0.01$\\
%   3C~401&  $59.60$  &$-24.77\pm 0.02$&$18.88\pm 0.31$&$22.32\pm 0.01$&$3.70\pm 0.04$&$0.18\pm 0.00$&$-85.91\pm 0.40$&$-0.05\pm 0.03$\\
%   3C~402&  $...$    &$-22.94\pm 0.00$&$1.84\pm 0.00$&$18.28\pm 0.00$&$2.86\pm 0.00$&$0.18\pm 0.00$&$34.29\pm 0.06$&$-0.15\pm 0.00$\\
%   3C~403&  $62.52$  &$-24.44\pm 0.05$&$7.98\pm 0.05$&$20.35\pm 0.05$&$4.56\pm 0.00$&$0.26\pm 0.01$&$36.68\pm 2.32$&$-0.13\pm 0.00$\\
%   3C~403.1&$...$    &$-22.73\pm 0.00$&$1.33\pm 0.00$&$18.01\pm 0.00$&$3.48\pm 0.01$&$0.19\pm 0.00$&$-27.94\pm 0.16$&$0.34\pm 0.01$\\
%   3C~405&  $...$    &$-22.98\pm 0.17$&$3.84\pm 0.13$&$19.32\pm 0.17$&$0.76\pm 0.00$&$0.21\pm 0.01$&$-16.97\pm 2.17$&$0.02\pm 0.00$\\
%   3C~410&  $...$    &$-25.08\pm 0.02$&$5.62\pm 0.13$&$19.79\pm 0.00$&$5.87\pm 0.20$&$0.16\pm 0.01$&$85.91\pm 0.82$&$0.05\pm 0.03$\\
%   3C~424&  $...$    &$-23.32\pm 0.01$&$7.58\pm 0.13$&$21.84\pm 0.00$&$6.81\pm 0.08$&$0.08\pm 0.00$&$84.81\pm 0.85$&$-0.07\pm 0.00$\\
%   3C~430&  $62.47$  &$-23.86\pm 0.00$&$3.67\pm 0.01$&$19.16\pm 0.00$&$4.06\pm 0.01$&$0.37\pm 0.00$&$-73.44\pm 0.06$&$0.00\pm 0.00$\\
%   3C~433&  $-21.16$ &$-24.28\pm 0.01$&$6.61\pm 0.08$&$19.93\pm 0.00$&$2.36\pm 0.04$&$0.41\pm 0.00$&$-29.51\pm 0.24$&$-0.39\pm 0.02$\\
%   3C~436&  $59.42$  &$-24.46\pm 0.00$&$4.87\pm 0.02$&$19.62\pm 0.00$&$2.91\pm 0.01$&$0.23\pm 0.00$&$11.80\pm 0.27$&$0.00\pm 0.02$\\
%   3C~438&  $...$    &$-25.07\pm 0.01$&$6.37\pm 0.03$&$19.80\pm 0.01$&$2.57\pm 0.02$&$0.07\pm 0.00$&$-16.52\pm 0.94$&$-0.03\pm 0.02$\\
%   3C~442&  $64.46$  &$-22.26\pm 0.00$&$1.55\pm 0.00$&$18.19\pm 0.00$&$1.28\pm 0.00$&$0.12\pm 0.00$&$-47.59\pm 0.17$&$-0.26\pm 0.00$\\
%   3C~445&  $...$    &$-22.21\pm 0.01$&$1.75\pm 0.00$&$19.17\pm 0.01$&$3.74\pm 0.36$&$0.15\pm 0.00$&$77.94\pm 0.00$&$0.13\pm 0.00$\\
%   3C~449&  $...$    &$-22.36\pm 0.00$&$1.16\pm 0.00$&$17.52\pm 0.00$&$1.55\pm 0.00$&$0.18\pm 0.00$&$-3.86\pm 0.08$&$-0.24\pm 0.00$\\
%   3C~452&  $...$    &$-23.75\pm 0.00$&$3.78\pm 0.01$&$19.41\pm 0.00$&$3.84\pm 0.01$&$0.28\pm 0.00$&$-74.87\pm 0.09$&$-0.07\pm 0.00$\\
%   3C~459&  $-21.86$ &$-24.61\pm 0.01$&$3.17\pm 0.04$&$19.20\pm 0.00$&$9.79\pm 0.14$&$0.05\pm 0.00$&$-61.31\pm 0.96$&$0.10\pm 0.02$\\
%   3C~465&  $...$    &$-24.09\pm 0.01$&$4.04\pm 0.02$&$18.80\pm 0.01$&$2.56\pm 0.01$&$0.19\pm 0.00$&$30.09\pm 0.11$&$0.02\pm 0.00$\\

% 3C~15 & ... & -24.33 & 8.41 & 18.86 & 6.10 & 0.07 & 19.33 & 0.11 \\ 
% 3C~17 & -21.51 & -24.19 & 4.25 & 17.52 & 7.49 & 0.23 & 20.94 & -0.21 \\ 
% 3C~20 & ... & -23.61 & 2.19 & 16.66 & 2.70 & 0.10 & -65.53 & -0.15 \\ 
% 3C~28 & -18.71 & -24.70 & 11.12 & 19.10 & 2.32 & 0.24 & -33.50 & -0.26 \\ 
% 3C~29 & -16.19 & -23.82 & 4.24 & 17.89 & 1.45 & 0.04 & -81.55 & 0.08 \\ 
% 3C~31 & ... & -23.29 & 1.72 & 16.46 & 1.67 & 0.12 & -32.98 & -0.01 \\ 
% 3C~33 & ... & -23.43 & 2.98 & 17.51 & 3.60 & 0.08 & -35.60 & -0.13 \\ 
% 3C~33.1 & -20.86 & -23.84 & 2.68 & 16.86 & 6.41 & 0.01 & 54.91 & 0.00 \\ 
% 3C~35 & ... & -24.07 & 8.38 & 19.11 & 4.79 & 0.28 & -66.34 & -0.02 \\ 
% 3C~52 & ... & -25.06 & 5.22 & 17.10 & 2.49 & 0.35 & 10.16 & -0.17 \\ 
% 3C~61.1 & -16.96 & -22.18 & 1.73 & 17.59 & 2.83 & 0.13 & -2.02 & 0.41 \\ 
% 3C~66B & ... & -23.35 & 2.93 & 17.56 & 2.39 & 0.07 & -59.24 & 0.00 \\ 
% 3C~71 & ... & ... & ... & ... & 3.08 & 0.39 & 44.44 & -0.37 \\ 
% 3C~75N & ... & -23.35 & 1.68 & 16.34 & 3.68 & 0.14 & -78.88 & 0.22 \\ 
% 3C~76.1 & ... & -22.28 & 1.31 & 16.88 & 2.95 & 0.16 & -48.12 & -0.08 \\ 
% 3C~79 & ... & -24.42 & 3.85 & 17.07 & 4.27 & 0.34 & 13.47 & 0.07 \\ 
% 3C~83.1 & ... & -23.98 & 2.74 & 16.78 & 2.03 & 0.26 & -9.97 & 0.03 \\ 
% 3C~84 & -19.25 & -22.20 & 1.88 & 17.74 & 1.26 & 0.20 & -68.41 & 0.28 \\ 
% 3C~88 & ... & -23.66 & 10.16 & 19.94 & 4.11 & 0.32 & -28.28 & 0.19 \\ 
% 3C~98 & ... & -22.93 & 2.24 & 17.39 & 3.88 & 0.17 & 53.26 & 0.00 \\ 
% 3C~105 & ... & -22.88 & 2.17 & 17.38 & 3.22 & 0.35 & 51.33 & -0.03 \\ 
% 3C~111 & -23.40 & -23.03 & 2.62 & 17.63 & 2.10 & 0.29 & 18.98 & 0.00 \\ 
% 3C~123 & ... & -25.26 & 15.44 & 19.25 & 4.55 & 0.08 & -80.73 & 0.06 \\ 
% 3C~129 & ... & -23.23 & 2.36 & 17.21 & 1.82 & 0.15 & -45.58 & 0.07 \\ 
% 3C~129.1 & ... & -23.59 & 3.08 & 17.42 & 1.68 & 0.06 & 87.02 & -0.02 \\ 
% 3C~130 & ... & -26.65 & 7.91 & 16.41 & 2.89 & 0.12 & -58.48 & -0.02 \\ 
% 3C~132 & ... & -24.93 & 6.48 & 17.70 & 3.52 & 0.21 & 16.13 & 0.00 \\ 
% 3C~133 & -23.11 & -24.63 & 4.43 & 17.17 & 8.65 & 0.12 & -10.48 & 0.00 \\ 
% 3C~135 & ... & -23.38 & 3.06 & 17.61 & 4.32 & 0.25 & -48.04 & 0.12 \\ 
% 3C~153 & ... & -24.68 & 5.90 & 17.75 & 4.37 & 0.12 & -68.55 & 0.00 \\ 
% 3C~165 & -18.70 & -24.24 & 3.63 & 17.13 & 2.54 & 0.15 & -0.01 & 0.19 \\ 
% 3C~166 & -21.02 & -24.66 & 24.89 & 20.89 & 8.83 & 0.10 & -83.89 & 0.00 \\ 
% 3C~171 & -18.47 & -23.62 & 2.87 & 17.23 & 2.59 & 0.09 & -60.45 & 0.00 \\ 
% 3C~173.1 & ... & -24.57 & 2.64 & 16.10 & 1.80 & 0.26 & 14.57 & 0.23 \\ 
% 3C~180 & ... & -24.63 & 9.77 & 18.89 & 2.89 & 0.45 & 31.33 & 0.68 \\ 
% 3C~184.1 & -20.66 & -23.16 & 2.02 & 16.93 & 5.89 & 0.27 & 44.52 & -0.17 \\ 
% 3C~192 & ... & -23.17 & 2.00 & 16.90 & 3.41 & 0.00 & -74.83 & 0.08 \\ 
% 3C~196.1 & ... & -25.79 & 41.00 & 20.84 & 3.73 & 0.32 & 53.34 & 0.00 \\ 
% 3C~197.1 & -18.78 & -23.62 & 4.19 & 18.05 & 5.03 & 0.00 & -4.98 & -0.18 \\ 
% 3C~198 & -18.53 & -22.55 & 3.14 & 18.50 & 6.44 & 0.13 & 70.70 & 0.00 \\ 
% 3C~213.1 & ... & -23.64 & 3.84 & 17.84 & 3.83 & 0.41 & -60.63 & -0.10 \\ 
% 3C~219 & -20.96 & -24.67 & 10.44 & 18.99 & 5.09 & 0.27 & -57.17 & -0.10 \\ 
% 3C~223 & ... & -23.88 & 6.88 & 18.87 & 5.18 & 0.19 & 65.25 & -0.57 \\ 
% 3C~223.1 & -16.66 & -24.66 & 15.79 & 19.90 & 9.73 & 0.42 & 40.18 & -0.41 \\ 
% 3C~227 & -22.43 & -22.66 & 2.48 & 17.89 & 2.68 & 0.15 & -3.34 & -0.22 \\ 
% 3C~234 & -23.71 & -23.36 & 2.95 & 17.56 & 1.59 & 0.08 & -74.91 & -0.12 \\ 
% 3C~236 & ... & -24.04 & 4.64 & 17.86 & 3.90 & 0.42 & 47.52 & 0.17 \\ 
% 3C~258 & ... & -20.11 & 1.19 & 18.84 & 3.26 & 0.27 & -35.04 & 0.00 \\ 
% 3C~264 & ... & -22.38 & 1.12 & 16.45 & 1.63 & 0.02 & -8.29 & 0.06 \\ 
% 3C~270 & ... & -22.63 & 1.49 & 16.81 & 1.96 & 0.27 & -22.24 & 0.00 \\ 
% 3C~272.1 & ... & -21.02 & 0.42 & 15.69 & 1.44 & 0.19 & -52.87 & 0.08 \\ 
% 3C~274 & -15.87 & -22.55 & 1.39 & 16.74 & 1.24 & 0.02 & -15.61 & 0.15 \\ 
% 3C~277.3 & ... & -23.42 & 3.19 & 17.67 & 2.51 & 0.07 & -21.38 & -0.06 \\ 
% 3C~284 & ... & -24.54 & 4.48 & 17.28 & 3.40 & 0.07 & 30.56 & 0.00 \\ 
% 3C~285 & ... & -23.61 & 7.30 & 19.28 & 3.13 & 0.36 & -57.18 & -0.19 \\ 
% 3C~287.1 & -23.16 & -24.14 & 5.28 & 18.04 & 5.94 & 0.15 & 34.92 & 0.00 \\ 
% 3C~288 & ... & -25.16 & 8.13 & 17.96 & 1.43 & 0.05 & -39.33 & -0.15 \\ 
% 3C~293 & ... & -24.40 & 18.45 & 20.50 & 4.15 & 0.46 & 58.41 & 0.00 \\ 
% 3C~296 & ... & -25.66 & 30.39 & 20.31 & 5.74 & 0.19 & 78.61 & 0.00 \\ 
% 3C~300 & ... & -23.52 & 2.84 & 17.32 & 3.10 & 0.31 & -51.10 & 0.00 \\ 
% 3C~303 & -15.05 & -24.94 & 27.64 & 20.83 & 4.00 & 0.12 & -16.06 & 0.18 \\ 
% 3C~305 & -18.97 & -24.42 & 14.02 & 19.88 & 5.96 & 0.26 & 68.91 & -0.11 \\ 
% 3C~310 & ... & -22.93 & 3.60 & 18.42 & 2.74 & 0.25 & 86.85 & -0.07 \\ 
% 3C~314.1 & ... & -22.96 & 3.67 & 18.43 & 3.31 & 0.40 & 70.99 & 0.06 \\ 
% 3C~315 & ... & -23.20 & 2.66 & 17.49 & 4.52 & 0.47 & 35.38 & -0.15 \\ 
% 3C~317 & -18.01 & -24.13 & 21.19 & 21.06 & 4.00 & 0.25 & 63.91 & -0.30 \\ 
% 3C~319 & ... & -23.62 & 6.76 & 19.10 & 7.34 & 0.22 & -42.45 & -0.18 \\ 
% 3C~321 & ... & -23.97 & 3.31 & 17.20 & 2.53 & 0.07 & -76.34 & 0.02 \\ 
% 3C~323.1 & -25.34 & -24.05 & 3.13 & 17.00 & 1.70 & 0.19 & 62.61 & 0.08 \\ 
% 3C~326 & ... & -22.99 & 2.17 & 17.26 & 3.47 & 0.45 & -72.75 & 0.00 \\ 
% 3C~332 & -23.61 & -23.37 & 3.20 & 17.73 & 1.72 & 0.01 & -53.83 & -0.09 \\ 
% 3C~338 & ... & -28.05 & 194.30 & 21.96 & 3.72 & 0.22 & 47.45 & 0.48 \\ 
% 3C~346 & -19.00 & -23.78 & 5.02 & 18.29 & 7.35 & 0.18 & -48.43 & 0.00 \\ 
% 3C~348 & ... & -24.25 & 10.13 & 19.35 & 1.06 & 0.32 & -59.47 & -0.05 \\ 
% 3C~349 & -20.41 & -23.49 & 3.37 & 17.72 & 3.54 & 0.44 & 21.21 & 0.12 \\ 
% 3C~353 & ... & -22.99 & 2.48 & 17.55 & 4.00 & 0.03 & 77.45 & 0.00 \\ 
% 3C~357 & ... & -24.98 & 11.34 & 18.86 & 5.34 & 0.29 & 83.67 & 0.00 \\ 
% 3C~371 & -23.07 & -23.37 & 2.31 & 17.02 & 3.81 & 0.07 & 71.56 & 0.07 \\ 
% 3C~379.1 & -19.24 & -24.96 & 6.31 & 17.61 & 2.98 & 0.10 & -45.01 & 0.00 \\ 
% 3C~381 & -19.10 & -23.77 & 2.84 & 17.07 & 3.62 & 0.18 & 64.63 & -0.05 \\ 
% 3C~382 & -23.40 & -24.29 & 4.66 & 17.61 & 5.81 & 0.31 & 88.99 & 0.00 \\ 
% 3C~386 & -19.48 & -22.73 & 1.76 & 17.07 & 2.50 & 0.13 & -75.63 & -0.05 \\ 
% 3C~388 & ... & -24.66 & 7.76 & 18.36 & 1.83 & 0.16 & 43.88 & -0.15 \\ 
% 3C~390.3 & -22.79 & -23.04 & 2.07 & 17.10 & 3.13 & 0.17 & 79.90 & -0.13 \\ 
% 3C~401 & ... & -24.77 & 18.88 & 20.18 & 3.70 & 0.18 & -85.91 & 0.34 \\ 
% 3C~402 & ... & -22.94 & 1.84 & 16.96 & 2.86 & 0.18 & 34.29 & 0.02 \\ 
% 3C~403 & ... & -24.44 & 7.98 & 18.64 & 4.56 & 0.26 & 36.68 & 0.05 \\ 
% 3C~403.1 & ... & -22.73 & 1.33 & 16.46 & 3.48 & 0.19 & -27.94 & -0.07 \\ 
% 3C~405 & -16.23 & -22.98 & 3.84 & 18.50 & 0.76 & 0.21 & -16.97 & 0.00 \\ 
% 3C~410 & -24.63 & -25.08 & 5.62 & 17.23 & 5.87 & 0.16 & 85.91 & -0.39 \\ 
% 3C~424 & -17.13 & -23.32 & 7.58 & 19.65 & 6.81 & 0.08 & 84.81 & 0.00 \\ 
% 3C~430 & ... & -23.86 & 3.67 & 17.53 & 4.06 & 0.37 & -73.44 & -0.03 \\ 
% 3C~433 & -21.16 & -24.28 & 6.61 & 18.40 & 2.36 & 0.41 & -29.51 & -0.26 \\ 
% 3C~436 & ... & -24.46 & 4.87 & 17.55 & 2.91 & 0.23 & 11.80 & 0.13 \\ 
% 3C~438 & ... & -25.07 & 6.37 & 17.53 & 2.57 & 0.07 & -16.52 & -0.24 \\ 
% 3C~442 & ... & -22.26 & 1.55 & 17.26 & 1.28 & 0.12 & -47.59 & -0.07 \\ 
% 3C~445 & -22.62 & -22.21 & 1.75 & 17.57 & 3.74 & 0.15 & 77.94 & 0.10 \\ 
% 3C~449 & ... & -22.36 & 1.16 & 16.54 & 1.55 & 0.18 & -3.86 & 0.02 \\ 
% 3C~452 & ... & -23.75 & 3.78 & 17.70 & 3.84 & 0.28 & -74.87 & 0.00 \\ 
% 3C~459 & -21.86 & -24.61 & 3.17 & 16.47 & 9.79 & 0.05 & -61.31 & -0.24 \\ 
% 3C~465 & ... & -24.09 & 4.04 & 17.51 & 2.56 & 0.19 & 30.09 & 0.00 \\ 
\enddata
\tablecomments{Properties of the best-fit 2-D \sersic model to each source:
Absolute magnitudes of the nucleus and host galaxy; 
scale-length (half-light radius) in kpc $R_e$; 
surface brightness at the scale-length $\mu$; 
\sersic index $n$; 
ellipticity $1-\frac{b}{a}$; 
position angle $\theta$ (relative to North); 
diskiness, $d$.
Notes: The following objects did not admit a complete or normal fit, as discussed in the main text: (a) 3C~71 is too extended to be properly constrained on either the NIC2 or WFPC2 chips; (b) 3C~258 -- values are presented as if the target lay at $z=0.165$, however it is likely that the source is actually at higher redshift.}
\end{deluxetable}



==> tab6.tex <==
% Table X: Optical data
\begin{deluxetable}{llll}
  \tabletypesize{\tiny}
  \tablecolumns{4}
  \tablewidth{0pc}
  \renewcommand{\arraystretch}{.6}
  \tablecaption{\label{tab-opt} Optical data from the WFPC2 archive}
  \tablehead{
  \colhead{Source} &
  \colhead{PROPOSID} & 
  \colhead{Filter} & 
  \colhead{exptime}}
\startdata
%  \input{/Users/floyd/3C/Work/idl/R_H}
3C~15	&	6348,5476	&	F555W,F702W 	&	600,280 \\
3C~17	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~20	&	5476		&	F702W		&	300 \\
3C~28	&	5476		&	F702W		&	280 \\
3C~29	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~31	&	6673,5476,6673	&	F555W,F702W,F814W&	460,280,460 \\
3C~33	&	5156		&	F702W		&	1700 \\
3C~33.1	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~35	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~52	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~61.1	&	6348,5476	&	F555W,F702W	&	600,300 \\
3C~66B	&	6673,5476,6673	&	F555W,F702W,F814W&	460,280,460 \\
3C~71	&	5754,5754,5754,5479&	F218W,F336W,F791W,F606W&2400,900,440,500 \\
3C~75	&	5476,5927	&	F702W,F791W	&	280,750 \\
3C~76.1	&	6967		&	F555W		&	600 \\
3C~79	&	5930,6776,5476	&	F300W,F675W,F702W&	1400,2260,280 \\
3C~83.1	&	5476		&	F702W		&	280 \\
3C~84	&	5476,6228,6228	&	F702W,F450W,F702W&	560,4700,5100 \\
3C~88	&	5476		&	F702W		&	280 \\
3C~98	&	5476		&	F702W		&	280 \\
3C~99	&	5476		&	F702W		&	300 \\
3C~111	&	5476,5931	&	F702W,F791W	&	280,8100 \\
3C~123	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~129	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~129.1&	6967,6363	&	F555W,F702W	&	600,460 \\
3C~130	&	6967		&	F555W		&	300 \\
3C~132	&	6348,5476	&	F555W,F702W	&	600,280 \\
3C~133	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~135	&	5476		&	F702W		&	280 \\
3C~153	&	5476		&	F702W		&	280 \\
3C~165	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~166	&	6348,5476	&	F555W,F702W	&	600,300 \\
3C~171	&	6967,5476	&	F555W,F702W	&	600,600 \\
3C~173.1&	5476		&	F702W		&	300 \\
3C~180	&	6967,5476,5476	&	F555W,F702W,F702W&	600,300,300 \\
3C~184.1&	5476		&	F702W		&	280, \\
3C~192	&	6348,5476,5476	&	F555W,F702W,F702W&	600,280,280 \\
3C~196.1&	5476		&	F702W		&	280 \\
3C~197.1&	5476		&	F702W		&	280 \\
3C~198	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~213.1&	6967,5476,5476	&	F555W,F702W,F702W&	600,300,300 \\
3C~219	&	6348,6776,5476	&	F555W,F675W,F702W&	600,2300,280 \\
3C~223	&	5476		&	F702W		&	280 \\
3C~223.1&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~227	&	6967,5476,5476	&	F555W,F702W,F702W&	600,560,560 \\
3C~234	&	6967,6776,5476	&	F555W,F675W,F702W&	1200,2260,280 \\
3C~236	&	6348,5476	&	F555W,F702W	&	600,560 \\
3C~258	&	5476,5476	&	F702W,F702W	&	300,300 \\
3C~264	&	5927,5479,5476	&	F791W,F606W,F702W&	750,500,280 \\
3C~270	&	5124,5476,5124	&	F675W,F702W,F791W&	2000,280,800 \\
3C~272.1&	5476,6094	&	F702W,F814W	&	280,520 \\
3C~274	&	5477p,6775,7274,8140,5476,5477,6775,7274,8140&	F555W,F606W,F606W,F606W,F702W,F814W,F814W,F814W,F814W	&	2400,520,520,320,280,2400,1480,480,480 \\
3C~277.3&	6348,5476	&	F555W,F702W	&	1000,600,560 \\
3C~284	&	5476		&	F702W		&	280 \\
3C~285	&	6967,5156	&	F555W,F702W	&	600,1200 \\
3C~287.1&	6776,5476	&	F675W,F702W	&	2300,280 \\
3C~288	&	5476		&	F702W		&	280 \\
3C~293	&	5476		&	F702W		&	280 \\
3C~296	&	5476		&	F702W		&	280 \\
3C~300	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~303	&	6348,5476	&	F555W,F702W	&	600,280 \\
3C~305	&	6967,5476	&	F555W,F702W	&	600,560 \\
3C~310	&	5476		&	F702W		&	280 \\
3C~314.1&	5476		&	F702W		&	280 \\
3C~315	&	5476		&	F702W		&	280 \\
3C~317	&	6810,5476,6810	&	F555W,F702W,F814W&	6200,280,6500 \\
3C~319	&	6967,5476	&	F555W,F702W,	&	600,280 \\
3C~321	&	5476		&	F702W		&	280 \\
3C~323.1&	5099		&	F606W		&	1800 \\
3C~326	&	6967,5476	&	F555W,F702W,	&	600,280 \\
3C~332	&	6348,5476	&	F555W,F702W	&	600,280 \\
3C~338	&	7265,5476	&	F555W,F702W	&	5200,280 \\
3C~346	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~348	&	5476		&	F702W		&	280 \\
3C~349	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~353	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~357	&	5476		&	F702W		&	280 \\
3C~371	&	6363,5476	&	F555W,F702W	&	240,560 \\
3C~379.1&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~381	&	5476		&	F702W		&	280 \\
3C~382	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~386	&	5476		&	F702W		&	280 \\
3C~388	&	5476		&	F702W		&	280 \\
3C~390.3&	5476		&	F702W		&	280 \\
3C~401	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~402	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~403	&	5476		&	F702W		&	280 \\
3C~403.1&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~405	&	5368,5104,5909	&	F555W,F622W,F814W& 	2700,1800,1000 \\
3C~410	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~424	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~430	&	6967,5476	&	F555W,F702W	&	600,280 \\
3C~433	&	5476		&	F702W		&	280 \\
3C~436	&	6967,6776,5476	&	F555W,F675W,F702W&	600,2260,280 \\
3C~438	&	6967,5476	&	F555W,F702W	&	600,300 \\
3C~442	&	5476,5927	&	F702W,F791W	&	280,750 \\
3C~445	&	6348,5476	&	F555W,F702W	&	280 \\
3C~449	&	5476		&	F702W		&	560 \\
3C~452	&	5476		&	F702W		&	280 \\
3C~459	&	6356,5476,6346	&	F606W,F702W,F814W&	600,280,800 \\
3C~465	&	6967,5476	&	F555W,F702W	&	600,280 \\
\enddata
\tablecomments{Optical (WFPC2) images for each sample were obtained from the MAST, or from Andr\'{e} Martel's website (see text). The table indicates the proposal ID for each image used, along with the filter for the observation, and the integration time.}
\end{deluxetable}



==> tab7.tex <==
% Table 8: COMPANIONS

\begin{deluxetable}{llllrllrr|ccccccccc}  
  \tabletypesize{\tiny}
  \tablecolumns{18}
  \tablewidth{0pc} 
  \renewcommand{\arraystretch}{.6}
  \tablecaption{\label{tab-companions} Companion Sources} 
  \tablehead{
    \colhead{Source} & \colhead{$N$} & 
    \colhead{$\alpha_{\mathrm J2000}$} & \colhead{$\delta_{\mathrm J2000}$} & 
    \colhead{$D$/arcsec} & \colhead{$H$} & \colhead{FWHM} &
    \colhead{Elong.} & \colhead{Ellip.} & 
    \colhead{Sh} & \colhead{TT} & \colhead{M} & \colhead{PM} & 
    \colhead{Maj} & \colhead{Min} & \colhead{Pt} & \colhead{Jet} & \colhead{DD}}
  \startdata
%    \input{/Users/floyd/3C/Work/idl/companions}
3C~15&      3& 00 37 04.05 & -01 09 05.5&16.57&19.21& 8.60&1.26&0.21 & ...&...&...&...&...& Y &...&...& Y   \\
3C~17&      3& 00 38 20.75 & -02 07 41.8& 6.73&22.43& 7.15&2.55&0.61 & ...&...&...& Y &...& Y &...&...&...  \\
3C~20&   $>9$& 00 43 09.67 & +52 03 30.5&18.31&17.80& 2.20&1.04&0.04 &  ? &...&...&...&...& Y & Y &...&...  \\
3C~28&   $>9$& 00 55 50.24 & +26 24 45.5&22.65&18.84& 4.31&1.04&0.04 & ...&...&...&...&...& Y &...& Y &...  \\
3C~29&      1& 00 57 35.33 & -01 23 37.4&23.63&24.04& 1.98&1.47&0.32 & ...&...&...&...&...&...&...&...&...  \\
3C~31&      3& 01 07 24.44 & +32 24 44.0&15.67&21.20& 2.18&1.28&0.22 & ...&...&...& Y & Y &...&...& Y &...  \\
3C~33&      0& ...         & ...        & ... & ... & ... & ...& ... & ...& Y &...&...&...&...&...& Y &...  \\
3C~33.1&    1& 01 09 44.11 & +73 11 54.4& 4.49&17.51& 4.87&1.99&0.50 & ...&...&...& Y & Y &...&...&...&...  \\
3C~35&      8& 01 12 01.93 & +49 28 44.2&15.93&17.81& 2.08&1.06&0.06 & ...&...&...& Y &...& Y & Y &...&...  \\
3C~52&   $>9$& 01 48 28.08 & +53 32 44.8& 6.60&18.66& 5.12&1.40&0.29 & ...&...&...&...&...& Y & Y & Y &...  \\
3C~61.1& $>9$& 02 22 36.07 & +86 19 07.7&11.73&18.10& 5.47&1.12&0.10 & ...& Y &...& Y & Y & Y & Y & Y &...  \\
3C~66B&     4& 02 23 11.54 & +42 59 23.1&16.55&19.52& 2.60&1.07&0.06 & ...&...&...& Y & Y &...& Y &...& Y   \\
3C~71&   $>9$& 02 42 41.38 & -00 00 49.4&17.70&18.06& 3.23&1.13&0.11 & ...&...&...&...&...& Y & Y &...&...  \\
3C~75N&     4& 02 57 43.63 & +06 02 31.5&18.89&18.74&12.54&2.69&0.63 & ...&...&...& Y & Y &...& Y &...&...  \\
3C~76.1&    5& 03 03 15.19 & +16 26 24.2& 9.65&19.99&17.36&2.24&0.55 & ...& Y &...&...&...& Y & Y & Y &...  \\
3C~79&      4& 03 10 00.19 & +17 05 57.8&12.64&16.96& 3.81&1.27&0.21 & ...&...& Y &...&...& Y &...&...&...  \\
3C~83.1& $>9$& 03 18 16.30 & +41 51 29.4&13.94&12.25& 9.67&4.85&0.79 & ...&...&...& Y & Y &...& Y & Y &...  \\
3C~84&   $>9$& 03 19 48.67 & +41 30 45.3&15.17&41.27& 2.57&1.06&0.05 & ...&...&...& Y & Y & Y & Y & Y &...  \\
3C~88&      3& 03 27 55.27 & +02 33 36.2&16.38&22.87& 2.10&1.53&0.35 &  ? & ? &...& ? & ? & ? & Y &...&...  \\
3C~98&      7& 03 58 55.20 & +10 25 51.0&19.75&18.24& 6.11&1.35&0.26 & ...&...&...& Y &...& Y &...&...&...  \\
3C~105&     2& 04 07 26.12 & +03 42 26.7&18.59&23.31& 4.01&1.39&0.28 & ...&...&...&...&...&...& Y &...&...  \\
3C~111&  $>9$& 04 18 21.84 & +38 01 37.8& 7.93&13.05&16.68&2.35&0.57 & ...&...&...&...&...&...& Y &...&...  \\
3C~123&     6& 04 37 03.79 & +29 40 08.0&22.21&19.95& 9.19&1.62&0.38 & ...& ? &...&...&...& Y & Y &...&...  \\
3C~129&  $>9$& 04 48 58.20 & +45 02 02.3&15.04&16.65& 2.42&1.10&0.09 & ...&...&...&...&...& Y & Y &...&...  \\
3C~129.1&$>9$& 04 50 07.22 & +45 03 28.7&17.17&17.66& 2.19&1.04&0.03 & ...&...&...&...&...&...& Y &...&...  \\
3C~130&  $>9$& 04 52 51.63 & +52 04 56.1& 7.69&18.58& 2.08&1.03&0.03 & ...&...&...&...&...&...& Y &...&...  \\
3C~132&  $>9$& 04 56 43.14 & +22 49 21.5&12.68&15.14&10.98&1.42&0.30 & ...&...&...& Y &...& Y & Y &...&...  \\
3C~133&     7& 05 02 58.44 & +25 16 25.3& 6.47&17.50& 3.89&2.08&0.52 & ...& Y &...& Y & Y &...& Y &...& Y   \\
3C~135&     7& 05 14 08.40 & +00 56 30.0&13.88&17.79& 8.85&1.15&0.13 & ...&...&...& Y & Y & Y &...&...&...  \\
3C~153&  $>9$& 06 09 31.79 & +48 04 14.1&17.60&13.82&11.51&2.55&0.61 & ...&...&...& Y &...& Y & Y &...&...  \\
3C~165&     9& 06 43 06.77 & +23 18 59.0&16.35&18.78& 2.18&1.12&0.11 & ...&...&...& Y &...& Y & Y &...&...  \\
3C~166&     1& 06 45 24.01 & +21 21 54.5&10.92&23.78& 2.75&1.63&0.39 & ...&...&...&...&...&...& Y &...& ?   \\
3C~171&     5& 06 55 14.67 & +54 08 56.9&11.15&19.76& 2.01&1.03&0.03 & ...& Y &...&...&...& Y & Y &...& Y   \\
3C~173.1&$>9$& 07 09 18.58 & +74 49 28.4&10.96&21.72& 5.39&1.92&0.48 & ...& Y &...&...&...& Y &...& Y &...  \\
3C~180&     9& 07 27 04.79 & -02 04 34.6&16.83&20.44&11.63&1.41&0.29 & ...& Y &...&...&...& Y & Y & Y &...  \\
3C~184.1&$>9$& 07 43 02.08 & +80 26 26.6&13.27&18.56& 9.88&1.74&0.43 &  ? & Y &...& Y &...& Y & Y &...&...  \\
3C~192&     5& 08 05 31.78 & +24 10 32.2&26.37&22.27& 9.01&2.52&0.60 & ...&...&...&...&...& Y & Y &...&...  \\
3C~196.1&   9& 08 15 28.14 & -03 08 24.0&12.15&19.34& 3.77&1.25&0.20 & ...& Y &...& Y &...& Y & Y & Y &...  \\
3C~197.1&   5& 08 21 32.46 & +47 02 39.5&18.77&21.59&11.68&2.23&0.55 & ...&...&...&...&...& Y &...&...&...  \\
3C~198&     1& 08 22 31.90 & +05 57 01.8&14.22&23.06& 6.68&2.60&0.62 & ...& Y &...&...&...& Y &...&...&...  \\
3C~213.1&   9& 09 01 04.85 & +29 01 56.4&16.30&21.34& 9.57&1.78&0.44 & ...& Y &...&...& Y & Y &...&...& 0   \\
3C~219&     5& 09 21 08.95 & +45 38 50.5&12.49&17.10&15.16&3.14&0.68 & ...&...&...& Y & Y & Y &...&...&...  \\
3C~223&  $>9$& 09 39 52.58 & +35 53 46.0&18.89&21.18& 4.15&3.30&0.70 & ...& Y &...&...& Y &...&...&...&...  \\
3C~223.1&   2& 09 41 25.02 & +39 44 46.7&15.59&21.37& 8.23&1.44&0.30 & ...& Y &...&...&...& Y &...& Y &...  \\
3C~227&  $>9$& 09 47 46.29 & +07 25 10.0&14.76&14.92&19.28&1.75&0.43 & ...& Y &...& Y &...& Y &...&...&...  \\
3C~234&  $>9$& 10 01 49.44 & +28 47 08.5&13.78&15.60& 2.28&1.13&0.11 & ...&...&...&...&...& Y &...&...& Y   \\
3C~236&     5& 10 06 01.52 & +34 54 15.9&18.21&22.27& 5.90&1.23&0.19 &  Y & Y &...&...&...& Y &...& Y &...  \\
3C~258&     6& 11 24 43.92 & +19 19 29.3&13.43&19.78& 5.22&1.46&0.31 & ...& Y & Y &...& Y & Y &...& Y &...  \\
3C~264&     1& 11 45 04.38 & +19 36 25.0&17.68&22.26& 2.25&1.07&0.07 & ...&...&...&...&...& Y & Y & Y & Y   \\
3C~270&     4& 12 19 23.48 & +05 49 40.9& 4.33&20.83& 2.34&1.10&0.09 & ...&...&...&...&...&...& Y & Y &...  \\
3C~272.1&   0& ...         & ...        & ... & ... & ... & ...& ... & ...&...&...&...&...&...& Y & Y &...  \\
3C~274&  $>9$& 12 30 48.62 & +12 23 32.3&17.69&16.26&10.39&1.18&0.15 & ...&...&...&...&...&...& Y &...& Y   \\
3C~277.3&   9& 12 54 12.23 & +27 37 26.0&10.40&19.66& 2.06&1.05&0.05 & ...& Y &...& Y &...& Y & Y &...& Y   \\
3C~284&  $>9$& 13 11 04.93 & +27 28 04.6& 9.22&20.26& 4.16&1.19&0.16 & ...& Y &...&...&...& Y &...&...&...  \\
3C~285&     3& 13 21 17.65 & +42 35 23.7&19.46&21.59& 9.41&1.62&0.38 & ...& Y &...&...& Y & Y &...& Y &...  \\
3C~287.1&   1& 13 32 53.46 & +02 00 48.9& 2.53&20.26& 3.33&1.15&0.13 & ...&...&...& Y &...& Y &...&...&...  \\
3C~288&     7& 13 38 49.41 & +38 51 13.2& 7.66&17.56& 4.82&1.54&0.35 & ...&...&...& Y &...& Y & Y &...&...  \\
3C~293&     6& 13 52 18.34 & +31 26 50.2&14.56&21.17& 7.68&1.57&0.36 & ...& Y & Y &...&...& Y &...& Y & Y   \\
3C~296&     1& 14 16 53.00 & +10 48 36.9&18.06&20.30& 2.12&1.03&0.03 & ...& Y &...&...&...&...& Y & Y &...  \\
3C~300&     3& 14 22 59.28 & +19 35 35.1&14.05&20.57&14.24&1.48&0.33 & ...& Y &...&...&...& Y &...&...&...  \\
3C~303&     5& 14 43 03.54 & +52 01 44.0&22.29&19.72& 2.07&1.07&0.06 & ...& Y &...& Y &...& Y & Y &...&...  \\
3C~305&     0& ...         & ...        & ... & ... & ... & ...& ... & ...& Y &...&...&...&...&...& Y &...  \\
3C~310&  $>9$& 15 04 56.92 & +26 00 47.6&22.62&17.44& 2.06&1.05&0.05 & ...& Y &...& Y & Y & Y & Y &...&...  \\
3C~314.1&   4& 15 10 24.33 & +70 45 46.4& 6.70&21.09& 2.09&1.08&0.07 & ...& Y &...&...& Y &...& Y &...&...  \\
3C~315&     7& 15 13 39.96 & +26 07 20.3&10.61&16.19& 5.56&1.09&0.09 & ...& Y &...& Y & Y & Y &...&...&...  \\
3C~317&     3& 15 16 44.84 & +07 01 22.9& 7.67&17.08& 4.45&1.17&0.15 & ...& Y &...& Y & Y & Y & Y &...&...  \\
3C~319&     4& 15 24 06.32 & +54 28 23.6&14.34&18.43& 8.60&3.23&0.69 & ...&...&...& Y & Y & Y & Y &...&...  \\
3C~321&  $>9$& 15 31 43.22 & +24 04 21.0&14.26&16.77& 6.14&1.26&0.20 & ...& Y & Y &...& Y & Y &...& Y &...  \\
3C~323.1&$>9$& 15 47 43.48 & +20 52 15.6&13.05&15.05&16.85&2.99&0.67 & ...&...&...&...&...& Y & Y &...&...  \\
3C~326&     8& 15 52 08.46 & +20 05 33.7&26.13&22.17& 6.17&1.34&0.26 & ...& Y &...&...& Y & Y & Y & Y &...  \\
3C~332&  $>9$& 16 17 42.48 & +32 22 32.8&14.17&15.59& 1.52&1.09&0.09 & ...&...&...& Y & Y &...&...&...&...  \\
3C~338&     4& 16 28 38.27 & +39 33 05.8&15.12& 8.38& 9.91&1.15&0.13 & ...&...&...& Y & Y & Y & Y & Y &...  \\
3C~346&     4& 16 43 48.69 & +17 15 48.1& 7.39&17.58& 7.60&1.29&0.22 & ...& Y & Y &...& Y & Y & Y & Y & Y   \\
3C~348&  $>9$& 16 51 08.16 & +04 59 33.9&13.57&17.95&25.97&1.38&0.28 & ...& Y &...& Y & Y & Y & Y & Y &...  \\
3C~349&     4& 16 59 28.20 & +47 02 59.6&15.76&20.32& 2.05&1.04&0.04 & ...& Y &...&...&...& Y & Y &...&...  \\
3C~353&     4& 17 20 28.18 & -00 58 40.5& 7.26&21.92& 2.19&1.18&0.15 & ...&...&...&...&...&...& Y &...&...  \\
3C~357&     5& 17 28 20.88 & +31 46 07.2&19.13&19.53&15.98&2.02&0.50 & ...& Y &...&...&...& Y &...& Y &...  \\
3C~371&  $>9$& 18 06 50.89 & +69 49 29.2&14.90&13.19&19.43&3.23&0.69 & ...&...&...&...& Y &...&...&...& Y   \\
3C~379.1&   3& 18 24 29.72 & +74 20 50.2&18.59&22.35& 5.21&2.59&0.61 &  Y &...&...&...&...& Y &...&...&...  \\
3C~381&     4& 18 33 46.80 & +47 27 05.4&15.30&18.03& 6.32&1.47&0.32 & ...& Y &...& Y & Y & Y & Y &...&...  \\
3C~382&  $>9$& 18 35 03.45 & +32 41 46.2&12.80&13.23& 2.12&2.00&0.50 & ...& Y &...&...&...& Y & Y &...&...  \\
3C~386&  $>9$& 18 38 26.71 & +17 11 59.3&16.29&16.90& 3.01&1.25&0.20 & ...&...&...&...&...&...& Y &...&...  \\
3C~388&  $>9$& 18 44 01.75 & +45 33 28.3&15.07&16.28& 7.09&1.40&0.28 & ...&...&...& Y & Y & Y & Y &...&...  \\
3C~390.3&$>9$& 18 42 08.87 & +79 46 14.9&14.74&13.81&16.95&2.32&0.57 &  Y &...&...&...&...& Y & Y &...&...  \\
3C~401&  $>9$& 19 40 25.18 & +60 41 40.6&11.93&17.76& 5.06&1.06&0.05 & ...& Y &...& Y & Y & Y & Y &...& Y   \\
3C~402&     3& 19 41 46.85 & +50 35 43.4&20.88&19.51& 2.05&1.07&0.07 & ...&...&...&...&...& Y & Y &...&...  \\
3C~403&  $>9$& 19 52 16.33 & +02 30 25.7&15.98&16.93& 1.94&1.06&0.05 & ...& Y &...&...&...& Y & Y & Y &...  \\
3C~403.1&$>9$& 19 52 31.25 & -01 17 15.5&12.67&17.46&25.82&3.48&0.71 & ...&...&...& Y & Y & Y & Y &...&...  \\
3C~405&  $>9$& 19 59 27.50 & +40 44 10.6& 4.24&17.15& 3.88&1.35&0.26 & ...&...& Y &...&...& Y & Y & Y &...  \\
3C~410&  $>9$& 20 20 06.96 & +29 42 11.2& 0.33&40.78& 5.59&1.10&0.09 & ...&...&...&...&...&...& Y &...&...  \\
3C~424&     5& 20 48 12.28 & +07 01 20.0& 8.52&22.91& 5.73&1.20&0.17 & ...& Y &...&...&...& Y & Y &...&...  \\
3C~430&  $>9$& 21 18 20.26 & +60 48 10.1&20.40&18.39& 4.12&1.08&0.08 & ...& Y &...&...&...&...& Y & Y &...  \\
3C~433&  $>9$& 21 23 44.60 & +25 04 28.5&14.04&15.65& 2.51&1.57&0.36 & ...& Y & Y &...& Y & Y & Y & Y &...  \\
3C~436&     7& 21 44 12.41 & +28 10 20.7&15.57&19.83&10.68&2.40&0.58 & ...& Y &...&...&...& Y & Y & Y &...  \\
3C~438&  $>9$& 21 55 52.47 & +38 00 33.5&12.63&19.01& 4.97&1.45&0.31 & ...& Y &...& Y &...& Y & Y & Y &...  \\
3C~442&     6& 22 14 46.14 & +13 50 20.8&18.85&47.01& 4.80&2.06&0.51 & ...&...&...& Y & Y &...& Y &...&...  \\
3C~445&  $>9$& 22 23 49.63 & -02 06 15.0& 8.55&13.94&22.86&4.28&0.77 & ...& Y &...&...&...& Y &...&...&...  \\
3C~449&     8& 22 31 20.02 & +39 21 25.3&18.77&21.35& 2.63&1.63&0.39 & ...&...&...& Y & Y & Y & Y & Y &...  \\
3C~452&  $>9$& 22 45 48.09 & +39 41 15.8&13.18&18.04&18.45&4.65&0.79 & ...& Y &...& Y &...&...& Y &...&...  \\
3C~459&     3& 23 16 35.30 & +04 05 11.3& 3.27&21.45& 8.17&1.41&0.29 & ...& Y &...&...&...&...&...&...&...  \\
3C~465&     4& 23 38 29.53 & +27 02 02.1&11.08&18.45&23.40&4.27&0.77 & ...&...&...& Y & Y & Y & Y &...&...  \\

%   3C~15&      3& 00 37 04.05 & -01 09 05.5&16.57&19.21&8.60&1.26&0.21\\
%   3C~17&      3& 00 38 20.75 & -02 07 41.8&6.73&22.43&7.15&2.55&0.61\\
%   3C~20&   $>9$& 00 43 09.67 & +52 03 30.5&18.31&17.80&2.20&1.04&0.04\\
%   3C~28&   $>9$& 00 55 50.24 & +26 24 45.5&22.65&18.84&4.31&1.04&0.04\\
%   3C~29&      1& 00 57 35.33 & -01 23 37.4&23.63&24.04&1.98&1.47&0.32\\
%   3C~31&      3& 01 07 24.44 & +32 24 44.0&15.67&21.20&2.18&1.28&0.22\\
%   3C~33&      0& ... & ... & ... & ... & ... & ... & ... \\
%   3C~33.1&    1& 01 09 44.11 & +73 11 54.4&4.49&17.51&4.87&1.99&0.50\\
%   3C~35&      8& 01 12 01.93 & +49 28 44.2&15.93&17.81&2.08&1.06&0.06\\
%   3C~52&   $>9$& 01 48 28.08 & +53 32 44.8&6.60&18.66&5.12&1.40&0.29\\
%   3C~61.1& $>9$& 02 22 36.07 & +86 19 07.7&11.73&18.10&5.47&1.12&0.10\\
%   3C~66B&     4& 02 23 11.54 & +42 59 23.1&16.55&19.52&2.60&1.07&0.06\\
%   3C~71&   $>9$& 02 42 41.38 & -00 00 49.4&17.70&18.06&3.23&1.13&0.11\\
%   3C~75N&     4& 02 57 43.63 & +06 02 31.5&18.89&18.74&12.54&2.69&0.63\\
%   3C~76.1&    5& 03 03 15.19 & +16 26 24.2&9.65&19.99&17.36&2.24&0.55\\
%   3C~79&      4& 03 10 00.19 & +17 05 57.8&12.64&16.96&3.81&1.27&0.21\\
%   3C~83.1& $>9$& 03 18 16.30 & +41 51 29.4&13.94&12.25&9.67&4.85&0.79\\
%   3C~84&   $>9$& 03 19 48.67 & +41 30 45.3&15.17&41.27&2.57&1.06&0.05\\
%   3C~88&      3& 03 27 55.27 & +02 33 36.2&16.38&22.87&2.10&1.53&0.35\\
%   3C~98&      7& 03 58 55.20 & +10 25 51.0&19.75&18.24&6.11&1.35&0.26\\
%   3C~105&     2& 04 07 26.12 & +03 42 26.7&18.59&23.31&4.01&1.39&0.28\\
%   3C~111&  $>9$& 04 18 21.84 & +38 01 37.8&7.93&13.05&16.68&2.35&0.57\\
%   3C~123&     6& 04 37 03.79 & +29 40 08.0&22.21&19.95&9.19&1.62&0.38\\
%   3C~129&  $>9$& 04 48 58.20 & +45 02 02.3&15.04&16.65&2.42&1.10&0.09\\
%   3C~129.1&$>9$& 04 50 07.22 & +45 03 28.7&17.17&17.66&2.19&1.04&0.03\\
%   3C~130&  $>9$& 04 52 51.63 & +52 04 56.1&7.69&18.58&2.08&1.03&0.03\\
%   3C~132&  $>9$& 04 56 43.14 & +22 49 21.5&12.68&15.14&10.98&1.42&0.30\\
%   3C~133&     7& 05 02 58.44 & +25 16 25.3&6.47&17.50&3.89&2.08&0.52\\
%   3C~135&     7& 05 14 08.40 & +00 56 30.0&13.88&17.79&8.85&1.15&0.13\\
%   3C~153&  $>9$& 06 09 31.79 & +48 04 14.1&17.60&13.82&11.51&2.55&0.61\\
%   3C~165&     9& 06 43 06.77 & +23 18 59.0&16.35&18.78&2.18&1.12&0.11\\
%   3C~166&     1& 06 45 24.01 & +21 21 54.5&10.92&23.78&2.75&1.63&0.39\\
%   3C~171&     5& 06 55 14.67 & +54 08 56.9&11.15&19.76&2.01&1.03&0.03\\
%   3C~173.1&$>9$& 07 09 18.58 & +74 49 28.4&10.96&21.72&5.39&1.92&0.48\\
%   3C~180&     9& 07 27 04.79 & -02 04 34.6&16.83&20.44&11.63&1.41&0.29\\
%   3C~184.1&$>9$& 07 43 02.08 & +80 26 26.6&13.27&18.56&9.88&1.74&0.43\\
%   3C~192&     5& 08 05 31.78 & +24 10 32.2&26.37&22.27&9.01&2.52&0.60\\
%   3C~196.1&   9& 08 15 28.14 & -03 08 24.0&12.15&19.34&3.77&1.25&0.20\\
%   3C~197.1&   5& 08 21 32.46 & +47 02 39.5&18.77&21.59&11.68&2.23&0.55\\
%   3C~198&     1& 08 22 31.90 & +05 57 01.8&14.22&23.06&6.68&2.60&0.62\\
%   3C~213.1&   9& 09 01 04.85 & +29 01 56.4&16.30&21.34&9.57&1.78&0.44\\
%   3C~219&     5& 09 21 08.95 & +45 38 50.5&12.49&17.10&15.16&3.14&0.68\\
%   3C~223&  $>9$& 09 39 52.58 & +35 53 46.0&18.89&21.18&4.15&3.30&0.70\\
%   3C~223.1&   2& 09 41 25.02 & +39 44 46.7&15.59&21.37&8.23&1.44&0.30\\
%   3C~227&  $>9$& 09 47 46.29 & +07 25 10.0&14.76&14.92&19.28&1.75&0.43\\
%   3C~234&  $>9$& 10 01 49.44 & +28 47 08.5&13.78&15.60&2.28&1.13&0.11\\
%   3C~236&     5& 10 06 01.52 & +34 54 15.9&18.21&22.27&5.90&1.23&0.19\\
%   3C~258&     6& 11 24 43.92 & +19 19 29.3&13.43&19.78&5.22&1.46&0.31\\
%   3C~264&     1& 11 45 04.38 & +19 36 25.0&17.68&22.26&2.25&1.07&0.07\\
%   3C~270&     4& 12 19 23.48 & +05 49 40.9&4.33&20.83&2.34&1.10&0.09\\
%   3C~272.1&   0& ... & ... & ... & ... & ... & ... & ... \\
%   3C~274&  $>9$& 12 30 48.62 & +12 23 32.3&17.69&16.26&10.39&1.18&0.15\\
%   3C~277.3&   9& 12 54 12.23 & +27 37 26.0&10.40&19.66&2.06&1.05&0.05\\
%   3C~284&  $>9$& 13 11 04.93 & +27 28 04.6&9.22&20.26&4.16&1.19&0.16\\
%   3C~285&     3& 13 21 17.65 & +42 35 23.7&19.46&21.59&9.41&1.62&0.38\\
%   3C~287.1&   1& 13 32 53.46 & +02 00 48.9&2.53&20.26&3.33&1.15&0.13\\
%   3C~288&     7& 13 38 49.41 & +38 51 13.2&7.66&17.56&4.82&1.54&0.35\\
%   3C~293&     6& 13 52 18.34 & +31 26 50.2&14.56&21.17&7.68&1.57&0.36\\
%   3C~296&     1& 14 16 53.00 & +10 48 36.9&18.06&20.30&2.12&1.03&0.03\\
%   3C~300&     3& 14 22 59.28 & +19 35 35.1&14.05&20.57&14.24&1.48&0.33\\
%   3C~303&     5& 14 43 03.54 & +52 01 44.0&22.29&19.72&2.07&1.07&0.06\\
%   3C~305&     0& ... & ... & ... & ... & ... & ... & ... \\
%   3C~310&  $>9$& 15 04 56.92 & +26 00 47.6&22.62&17.44&2.06&1.05&0.05\\
%   3C~314.1&   4& 15 10 24.33 & +70 45 46.4&6.70&21.09&2.09&1.08&0.07\\
%   3C~315&     7& 15 13 39.96 & +26 07 20.3&10.61&16.19&5.56&1.09&0.09\\
%   3C~317&     3& 15 16 44.84 & +07 01 22.9&7.67&17.08&4.45&1.17&0.15\\
%   3C~319&     4& 15 24 06.32 & +54 28 23.6&14.34&18.43&8.60&3.23&0.69\\
%   3C~321&  $>9$& 15 31 43.22 & +24 04 21.0&14.26&16.77&6.14&1.26&0.20\\
%   3C~323.1&$>9$& 15 47 43.48 & +20 52 15.6&13.05&15.05&16.85&2.99&0.67\\
%   3C~326&     8& 15 52 08.46 & +20 05 33.7&26.13&22.17&6.17&1.34&0.26\\
%   3C~332&  $>9$& 16 17 42.48 & +32 22 32.8&14.17&15.59&1.52&1.09&0.09\\
%   3C~338&     4& 16 28 38.27 & +39 33 05.8&15.12&8.38&9.91&1.15&0.13\\
%   3C~346&     4& 16 43 48.69 & +17 15 48.1&7.39&17.58&7.60&1.29&0.22\\
%   3C~348&  $>9$& 16 51 08.16 & +04 59 33.9&13.57&17.95&25.97&1.38&0.28\\
%   3C~349&     4& 16 59 28.20 & +47 02 59.6&15.76&20.32&2.05&1.04&0.04\\
%   3C~353&     4& 17 20 28.18 & -00 58 40.5&7.26&21.92&2.19&1.18&0.15\\
%   3C~357&     5& 17 28 20.88 & +31 46 07.2&19.13&19.53&15.98&2.02&0.50\\
%   3C~371&  $>9$& 18 06 50.89 & +69 49 29.2&14.90&13.19&19.43&3.23&0.69\\
%   3C~379.1&   3& 18 24 29.72 & +74 20 50.2&18.59&22.35&5.21&2.59&0.61\\
%   3C~381&     4& 18 33 46.80 & +47 27 05.4&15.30&18.03&6.32&1.47&0.32\\
%   3C~382&  $>9$& 18 35 03.45 & +32 41 46.2&12.80&13.23&2.12&2.00&0.50\\
%   3C~386&  $>9$& 18 38 26.71 & +17 11 59.3&16.29&16.90&3.01&1.25&0.20\\
%   3C~388&  $>9$& 18 44 01.75 & +45 33 28.3&15.07&16.28&7.09&1.40&0.28\\
%   3C~390.3&$>9$& 18 42 08.87 & +79 46 14.9&14.74&13.81&16.95&2.32&0.57\\
%   3C~401&  $>9$& 19 40 25.18 & +60 41 40.6&11.93&17.76&5.06&1.06&0.05\\
%   3C~402&     3& 19 41 46.85 & +50 35 43.4&20.88&19.51&2.05&1.07&0.07\\
%   3C~403&  $>9$& 19 52 16.33 & +02 30 25.7&15.98&16.93&1.94&1.06&0.05\\
%   3C~403.1&$>9$& 19 52 31.25 & -01 17 15.5&12.67&17.46&25.82&3.48&0.71\\
%   3C~405&  $>9$& 19 59 27.50 & +40 44 10.6&4.24&17.15&3.88&1.35&0.26\\
%   3C~410&  $>9$& 20 20 06.96 & +29 42 11.2&0.33&40.78&5.59&1.10&0.09\\
%   3C~424&     5& 20 48 12.28 & +07 01 20.0&8.52&22.91&5.73&1.20&0.17\\
%   3C~430&  $>9$& 21 18 20.26 & +60 48 10.1&20.40&18.39&4.12&1.08&0.08\\
%   3C~433&  $>9$& 21 23 44.60 & +25 04 28.5&14.04&15.65&2.51&1.57&0.36\\
%   3C~436&     7& 21 44 12.41 & +28 10 20.7&15.57&19.83&10.68&2.40&0.58\\
%   3C~438&  $>9$& 21 55 52.47 & +38 00 33.5&12.63&19.01&4.97&1.45&0.31\\
%   3C~442&     6& 22 14 46.14 & +13 50 20.8&18.85&47.01&4.80&2.06&0.51\\
%   3C~445&  $>9$& 22 23 49.63 & -02 06 15.0&8.55&13.94&22.86&4.28&0.77\\
%   3C~449&     8& 22 31 20.02 & +39 21 25.3&18.77&21.35&2.63&1.63&0.39\\
%   3C~452&  $>9$& 22 45 48.09 & +39 41 15.8&13.18&18.04&18.45&4.65&0.79\\
%   3C~459&     3& 23 16 35.30 & +04 05 11.3&3.27&21.45&8.17&1.41&0.29\\
%   3C~465&     4& 23 38 29.53 & +27 02 02.1&11.08&18.45&23.40&4.27&0.77\\
\enddata
\tablecomments{Number and properties of companion sources for each 3CR target:
3CR number; 
Number of companions on NIC2 image;
Coordinates of brightest companion source;
Distance (arcsec) of brightest companion from radio source;
H-band absolute magnitude of brightest secondary; 
Diameter (FWHM) of secondary;
Elongation (if resolved);
Ellipticity (if resolved). 
The right-hand side of the table lists the presence of various types of artefact ('Y'): 
Shells; tidal tails; mergers; pre-mergers; major companion sources; minor companion sources; unresolved point-like companion sources; jets; dust disks. See the main test for a fuller description of each category. A questionmark '?' implies the presence of the artifact is suggested but cannot be confirmed categorically.
%Notes on morphological disturbance, and environment of the host galaxy.
%\tablerefs{\citet{dekoff+96} and references therein; 
%\citet{martel+99} and references therein;
%\citet{spinrad+85} - updated values were taken from the 
NASA Extragalactic Database (NED).}
\end{deluxetable}



==> tab8.tex <==
% Table 7: COLOURS
\begin{deluxetable}{lrrr}
  \tabletypesize{\tiny}
  \tablecolumns{4}
  \tablewidth{0pc}
  \renewcommand{\arraystretch}{.6}
  \tablecaption{\label{tab-col} Host galaxy $R-H$ colors}
  \tablehead{
  \colhead{Source} &
  \colhead{$R^{a}$} & 
  \colhead{$H$} & 
  \colhead{$R-H$}}
\startdata
%  \input{/Users/floyd/3C/Work/idl/R_H}
3c15 &	16.84 &	13.55 &	3.29 \\
3c29 &	16.53 &	12.89 &	3.64 \\
3c31 &	13.78 &	11.18 &	2.60 \\
3c35 &	16.84 &	13.68 &	3.16 \\
3c66B &	14.38 &	11.72 &	2.66 \\
3c75N &	14.22 &	12.07 &	2.15 \\
3c83.1 &13.92 &	11.53 &	2.39 \\
3c84 &	13.50 &	12.45 &	1.05 \\
3c88 &	15.92 &	12.23 &	3.68 \\
3c98 &	15.26 &	13.03 &	2.23 \\
3c111 &	17.12 &	14.83 &	2.29 \\
3c198 &	17.64 &	15.58 &	2.06 \\
3c227 &	16.21 &	15.61 &	0.60 \\
3c236 &	17.62 &	14.54 &	3.08 \\
3c264 &	14.17 &	12.55 &	1.62 \\
3c270 &	11.75 &	 9.98 & 1.77 \\
3c272.1&10.11 &  9.75 & 0.36 \\
3c274 &	10.61 &	 8.84 &	1.77 \\
3c277.3&17.57 & 14.81 & 2.76 \\
3c293 &	17.04 &	12.35 &	4.69 \\
3c296 &	14.05 &	 9.58 &	4.47 \\
3c305 &	15.34 &	12.13 &	3.21 \\
3c310 &	17.05 &	14.26 &	2.79 \\
3c317 &	16.16 &	12.06 &	4.10 \\
3c321 &	17.67 &	14.58 &	3.09 \\
3c326 &	17.72 &	15.35 &	2.37 \\
3c338 &	15.95 &	 7.70 &	8.25 \\
3c353 &	16.00 &	13.08 &	2.92 \\
3c371 &	14.96 &	13.64 &	1.32 \\
3c382 &	14.34 &	13.03 &	1.31 \\
3c386 &	13.26 &	12.01 &	1.25 \\
3c388 &	18.04 &	13.75 &	4.29 \\
3c390.3&15.38 & 14.25 & 1.13 \\
3c402 &	14.30 &	12.36 &	1.94 \\
3c403 &	16.10 &	13.04 &	3.06 \\
3c403.1&16.36 & 14.61 & 1.75 \\
3c430 &	17.17 &	13.67 &	3.50 \\
3c442 &	15.39 &	13.28 &	2.11 \\
3c445 &	15.27 &	15.09 &	0.18 \\
3c449 &	14.10 &	12.29 &	1.81 \\
3c452 &	17.12 &	14.44 &	2.68 \\
3c465 &	14.79 &	11.70 &	3.09 \\
\enddata
\tablecomments{Approximate $R-H$ colours for the sources based on $R$-band fluxes at a 20~kpc aperture.}
\tablerefs{$^{a}$~\citet{martel+99}.}
\end{deluxetable}

